Transgression forms as source for topological gravity and Chern-Simons-Higgs theories

Two main gauge invariant off-shell models are studied in this Thesis. I) Poincare-invariant topological gravity in even dimensions is formulated as a transgression field theory whose gauge connections are associated to linear and nonlinear realizations of the Poincare group ISO(d-1,1). The resulting theory is a gauged Wess-Zumino-Witten model whereby the transition functions relating gauge fields belong to the coset ISO(d-1,1)/SO(d-1,1). The supersymmetric extension leads to topological supergravity in two dimensions starting from a transgression field theory for the super-Poincare group in three dimensions. The construction is extended to a three-dimensional Chern-Simons theory of gravity invariant under the Maxwell algebra, where the corresponding Maxwell gauged Wess-Zumino-Witten model is obtained. II) dimensional reduction of Chern-Simons theories with arbitrary gauge group in a formalism based on equivariant principal bundles is considered. For the classical gauge groups the relations between equivariant principal bundles and quiver bundles is clarified, and show that the reduced quiver gauge theories are all generically built on the same universal symmetry breaking pattern. The reduced model is a novel Chern-Simons-Higgs theory consisting of a Chern-Simons term valued in the residual gauge group plus a higher order gauge and diffeomorphism invariant coupling of Higgs fields with the gauge fields. The moduli spaces of solutions provide in some instances geometric representations of certain quiver varieties as moduli spaces of flat invariant connections. In the context of dimensional reductions involving non-compact gauge groups, the reduction of five-dimensional supergravity induce novel couplings between gravity and matter. The resulting model is regarded as to a quiver gauge theory of AdS(3)xU(1) gravity involving a non-minimal coupling to scalar Higgs fermion fields.

==> Background.tex <==


\chapter{Mathematical Background}
\label{ch:background}

In order to describe gauge theories in a rigorous way it is necessary to
introduce the concept of \textit{Fiber Bundle}. A fiber bundle can be seen as a topological space which locally is the product of two manifolds. In the case when the product is also globally defined, the fiber bundle is said to be trivial. 

This mathematical concept is of vital importance in the construction of gauge theories. For this reason, a general, however not complete, description will be given through this chapter. For a more detailed analysis, see the books Ref.\cite{Nakahara} and Ref.\cite{deAz95}.

\section{Fiber Bundles}

\begin{definition}
A fiber bundle is composed by the set $\left\{  \mathcal{E},\mathcal{M}%
,\mathcal{F},\pi\right\}  $ where $\mathcal{E},\mathcal{M},\mathcal{F}$ are
topological spaces and $\pi:\mathcal{E}\rightarrow\mathcal{M}$ is a continuous
and surjective projection map. $\mathcal{E}$ is referred as to the total
space, $\mathcal{M}$ is the base space and $\mathcal{F}$ is the fiber.
\end{definition}

\begin{definition}
The local triviality condition $\varphi$ consists in the requirement that for
each $x\in\mathcal{M}$ there exist an open set $U$ such that
$\pi^{-1}\left(  U\right)  $ is homeomorphic to the direct product
$U\times\mathcal{F}$. The homeomorphism $\varphi:\pi^{-1}\left(  U\right)
\rightarrow U\times\mathcal{F}$ is such that the following diagram commutes,

\begin{figure}[here]
\centering
\begin{tikzcd}[column sep=6em,row sep=6em]
\pi^{-1}(U) \arrow[]{r}{\varphi}\arrow[]{d}{\pi}
&U \times F \arrow[]{dl}{\mathrm{proj}_1}\\
U&
\end{tikzcd}
\caption{Local Trivialization} \label{lotr}
\end{figure}
where $\mathrm{proj}_{1}$ denotes the standard projection map
$\mathrm{proj}_{1}:U\times\mathcal{F}\rightarrow\mathcal{F}$.
\end{definition}

Let $\left\{  U_{\alpha}\right\}  $ be an open covering of $\mathcal{M}$ in
such a way that $\bigcup\limits_{\alpha}U_{\alpha}=\mathcal{M}$. Each open
$U_{\alpha}$ has a homeomorphism $\varphi_{\alpha}$ associated. The set
$\left\{  U_{\alpha},\varphi_{\alpha}\right\}  $ corresponds to a
\textit{local trivialization} of the fiber bundle. Thus, for each
$x\in\mathcal{M}$ the pre-image $\pi^{-1}\left(  x\right)  $ is homeomorphic to
$\mathcal{F}$ and it will be called \textit{the fiber in} $x$. throughout
this thesis it will be assumed that the base space $\mathcal{M}$ is connected
so that the local triviality conditions is always fulfilled.

\subsection{Transitions Functions}

In order to describe the fiber bundle completely in terms of the local
trivializations $\left\{  U_{\alpha},\varphi_{\alpha}\right\}  $ it is
necessary to find juncture conditions in the non-empty overlaps between
different open sets $U$. Given two opens $U_{\alpha}$ and $U_{\beta}$ with
non-empty overlaps $U_{\alpha}\cap U_{\beta}\neq\varnothing$, they respective
homeomorphisms will, in general, map $\pi^{-1}\left(  U_{\alpha}\cap U_{\beta
}\right)  $ to $\left(  U_{\alpha}\cap U_{\beta}\right)  \times\mathcal{F}$ in
a different way%
\begin{align*}
\varphi_{\alpha} &  :\pi^{-1}\left(  U_{\alpha}\cap U_{\beta}\right)
\rightarrow\left(  U_{\alpha}\cap U_{\beta}\right)  \times\mathcal{F},\\
\varphi_{\beta} &  :\pi^{-1}\left(  U_{\alpha}\cap U_{\beta}\right)
\rightarrow\left(  U_{\alpha}\cap U_{\beta}\right)  \times\mathcal{F},
\end{align*}
or more explicitly%
\begin{align*}
\varphi_{\alpha}\left(  p\right)   &  =\left(  \pi\left(  p\right)
,y_{\alpha}\left(  p\right)  \right)  =\left(  x,y_{\alpha}\left(  p\right)
\right)  ,\\
\varphi_{\beta}\left(  p\right)   &  =\left(  \pi\left(  p\right)  ,y_{\beta
}\left(  p\right)  \right)  =\left(  x,y_{\beta}\left(  p\right)  \right)  ,
\end{align*}
where $x\in U_{\alpha}\cap U_{\beta}$, $y_{\alpha}\in\mathcal{F}$. This
induces the following
\begin{definition}
the composite map of $\varphi_{\alpha}$ and $\varphi_{\beta}^{-1}$ is
\begin{equation*}
\varphi_{\alpha}\circ\varphi_{\beta}^{-1}:\left(  U_{\alpha}\cap U_{\beta
}\right)  \times\mathcal{F}\rightarrow\left(  U_{\alpha}\cap U_{\beta}\right)
\times\mathcal{F},
\end{equation*}
or in a more explicit way%
\begin{equation*}
\varphi_{\alpha}\circ\varphi_{\beta}^{-1}\left(  x,y_{\beta}\right)  =\left(
x,\tau_{\alpha\beta}\left(  x\right)  y_{\beta}\right)  ,
\end{equation*}
where $\tau_{\alpha\beta}\left(  x\right)  $ corresponds to a continuous
left-acting operator over $\mathcal{F}$. The mappings $\tau_{\alpha\beta
}\left(  x\right)  :\mathcal{F}\rightarrow\mathcal{F}$ are called the
transitions functions and satisfy the following properties
\begin{enumerate}
\item $\tau_{\alpha\alpha}\left(  x\right)  =\mathrm{I}_{\mathcal{F}},$
\item $\tau_{\alpha\beta}\left(  x\right)  =\tau_{\beta\alpha}^{-1}\left(
x\right)  ,$
\item $\tau_{\alpha\gamma}\left(  x\right)  =\tau_{\alpha\beta}\left(
x\right)  \tau_{\beta\gamma}\left(  x\right)  .$
\end{enumerate}
\end{definition}

The last condition holds in the case $U_{\alpha}\cap U_{\beta}\cap U_{\gamma
}\neq\varnothing$ and is called the co-cycle condition. These three properties
implies that the transition functions $\tau$ form a group; the structure group
$\mathcal{G}$%
\begin{equation}
\tau_{\alpha\beta}:U_{\alpha}\cap U_{\beta}\rightarrow\mathcal{G}.%
\end{equation}

In the case of a \textit{smooth fiber bundle }($\mathcal{E},\mathcal{M}%
,\mathcal{F}$ differentiable manifolds and, $\pi,\varphi$ smooth maps),
$\mathcal{G}$ corresponds to a \textit{Lie group}. Throughout this thesis only
this kind of fiber bundle are considered. Note that the transition function
were chosen acting by the left, but this is only a matter of convention. In
principle, it is possible to define the \textit{right action }of a group over
the fiber and therefore inducing the right action over the whole bundle.

\begin{definition}
Let $g$ be an element of a symmetry group $\mathcal{G}$. We denote the right
action of $\mathcal{G}$ over the fibre $\mathcal{F}$ as%
\begin{equation*}
y_{\alpha}^{\prime}\left(  p\right)  =y_{\beta}\left(  p\right)  g.
\end{equation*}
Let $p,p^{\prime}$ be two point of the fiber bundle. It will be said that%
\begin{equation*}
p^{\prime}=pg
\end{equation*}
if the following conditions are satisfied%
\begin{align*}
\pi\left(  pg\right)   &  =\pi\left(  p\right)  ,\\
y_{\beta}\left(  pg\right)   &  =y_{\beta}\left(  p\right)  g.
\end{align*}
\end{definition}

The induced action over the bundle is independent of the homeomorphism
$\varphi$ and therefore of the choosing of $y_{\alpha}$. In fact, since%
\begin{equation*}
y_{\alpha}\left(  p\right)  =\tau_{\alpha\beta}\left(  x\right)  y_{\beta
}\left(  p\right)
\end{equation*}
it follows,%
\begin{align*}
y_{\alpha}\left(  pg\right)   &  =\tau_{\alpha\beta}\left(  x\right)
y_{\beta}\left(  pg\right)  ,\\
&  =\tau_{\alpha\beta}\left(  x\right)  y_{\beta}\left(  p\right)  g,\\
&  =y_{\alpha}\left(  p\right)  g.
\end{align*}

The existence of the left action $L_{g}$ and the right action $R_{g}$ of an
element $g\in\mathcal{G}$ acting on the bundle suggest the choosing of a
particularly elegant structure: the \textit{principal bundle}

\begin{definition}
A principal bundle is a fiber bundle in which
\begin{enumerate}
\item The fiber $\mathcal{F}$,
\item The set of transitions functions $\left\{  \tau_{\alpha\beta}\right\}  $,
\item The structure group $\mathcal{G}$ acting on the right, 
\end{enumerate}
\end{definition}
\textit{corresponds to the same Lie group} $\mathcal{G}$.

As it will be seen later, this kind of fiber bundle is the fundamental block
in the construction of gauge theories. In general, principal bundles are
denoted by $\mathcal{P}$ instead of $\mathcal{E}$ and of course the fiber
$\mathcal{F}$ is in this case denoted by $\mathcal{G}$.

\subsection{Local sections}

\begin{definition}
given the open covering $\left\{  U_{\alpha}\right\}  $ for $\mathcal{M}$ it
is possible to define a local section $\sigma_{\alpha}$ as the map%
\begin{equation*}
\sigma_{\alpha}:U_{\alpha}\longrightarrow\mathcal{P},%
\end{equation*}
such that $\forall x\in U_{\alpha}$
\begin{equation*}
\pi\circ\sigma_{\alpha}\left(  x\right)  =x.
\end{equation*}

\end{definition}

A section $\sigma_{\alpha}$ and the local homeomorphism $\varphi_{\alpha}%
:\pi^{-1}\left(  U_{\alpha}\right)  \rightarrow U_{\alpha}\times\mathcal{G}$
are intimately related. In fact, given a local trivialization $\varphi
_{\alpha}$ induces a particularly local section called \textit{natural section
}%
\begin{equation*}
\sigma_{\alpha}\left(  x\right)  =\varphi_{\alpha}^{-1}\left(  x,e\right),
\end{equation*}
where $e$ is the identity element of $\mathcal{G}$. The inverse affirmation
it is also true: a section induces a reciprocal local homeomorphism $\varphi$.
Thus, let $y_{\alpha}:\pi^{-1}\left(  U_{\alpha}\right)  \rightarrow
\mathcal{G}$ be the map such that%
\begin{equation}
\sigma_{\alpha}\left(  x\right)  y_{\alpha}\left(  p\right)  =p, \label{ch2.2}%
\end{equation}
where $y_{\alpha}\left(  p\right)  \in\mathcal{G}$ is acting by the right over
the point $\sigma_{\alpha}\left(  x\right)  $. Note that $\sigma_{\alpha
}\left(  x\right)  =p\left[  y_{\alpha}\left(  p\right)  \right]  ^{-1}$ it
does not depend on $p$. In fact, let $p^{\prime}=pg$ then%
\begin{align*}
p^{\prime}\left[  y_{\alpha}\left(  p^{\prime}\right)  \right]  ^{-1}  &
=pg\left[  y_{\alpha}\left(  pg\right)  \right]  ^{-1},\\
&  =pgg^{-1}\left[  y_{\alpha}\left(  p\right)  \right]  ^{-1},\\
&  =p\left[  y_{\alpha}\left(  p\right)  \right]  ^{-1}.
\end{align*}
Thus, it is possible to define
\begin{equation*}
\varphi_{\alpha}\left(  p\right)  =\left(  x,y_{\alpha}\left(  p\right)
\right),
\end{equation*}
where the condition eq.$\left(  \ref{ch2.2}\right)  $ implies that
$\sigma_{\alpha}\left(  x\right)  =\varphi_{\alpha}^{-1}\left(  x,e\right)  $.

Given two local sections $\sigma_{\alpha}$ and $\sigma_{\beta}$ over
$U_{\alpha}\cap U_{\beta}$, it is possible to show that they are related by the transition functions
$\tau_{\alpha\beta}:U_{\alpha}\cap U_{\beta}\rightarrow\mathcal{G}$. Let
$\sigma_{\alpha}$ and $\sigma_{\beta}$ be natural sections. Then, using eq$\left(
\ref{ch2.2}\right)  $ it follows%
\begin{equation*}
\sigma_{\alpha}\left(  x\right)  y_{\alpha}\left(  p\right)  =\sigma_{\beta
}\left(  x\right)  y_{\beta}\left(  p\right)  ,
\end{equation*}
but
\begin{equation*}
y_{\alpha}(p)=\tau_{\alpha \beta}(x) y_{\beta}(p),
\end{equation*}
therefore,
\begin{align*}
\sigma_{\alpha}\left(  x\right)  y_{\alpha}\left(  p\right)   &
=\sigma_{\alpha}\left(  x\right)  y_{\alpha}\left(  p\right)  \left[
y_{\beta}\left(  p\right)  \right]  ^{-1},\\
&  =\sigma_{\alpha}\left(  x\right)  \tau_{\alpha\beta}\left(  x\right) .
\end{align*}

\subsection{Symmetry group $\mathcal{G}$}

Since in the case of principal bundles the fiber $\mathcal{F}$ coincides with
the structure group $\mathcal{G}$, it is fair to precise at this point some important
features. Throughout this thesis the concepts of \textit{Lie algebra} and
\textit{Lie group} will be used interchangeably. 
Since $\mathcal{G}$ corresponds to a Lie group, it posses a manifold
structure. So, it is possible to define the \textit{tangent} space
$\mathrm{T}_{p}\left(  \mathcal{G}\right)  $ as the set of tangent vectors of
$\mathcal{M}$ at the point $p$. In particular, the Lie algebra $\mathfrak{g}$ associated to
$\mathcal{G}$ corresponds to the tangent space of the identity element
$\mathrm{T}_{e}\left(  \mathcal{G}\right)  $. The tangent space $\mathrm{T}_{e}\left(  \mathcal{G}\right)  $ has vector
space structure so if $\left\{  \mathrm{T}_{A}\right\}  $ is a basis for
$\mathrm{T}_{e}\left(  \mathcal{G}\right)  =\mathfrak{g}$; then%
\begin{equation}
\left[  \mathrm{T}_{A},\mathrm{T}_{B}\right]  =C_{AB}^{~~C}\mathrm{T}%
_{C},\label{pr1}%
\end{equation}
where $C_{AB}^{~~C}$ are known as the structure constants which satisfy%
\begin{equation*}
C_{AB}^{~~C}=-C_{BA}^{~~C},
\end{equation*}
and the \textit{Jacobi identity}%
\begin{equation*}
C_{AB}^{~~C}C_{CD}^{~~E}+C_{DA}^{~~C}C_{CB}^{~~E}+C_{BD}^{~~C}C_{CA}^{~~E}=0.
\end{equation*}
The commutator eq.$\left(  \ref{pr1}\right)  $ induce the notion of commutator
of differential forms valued in the Lie algebra $\mathfrak{g}$. Let $P$ and $Q$ be a $p$ and a
$q-$form respectively, defined over a manifold $\mathcal{X}$ and taking values in
the Lie algebra $\mathfrak{g}$, i.e.,%
\begin{align*}
P &  =P^{A}\mathrm{T}_{A},\\
Q &  =Q^{B}\mathrm{T}_{B},
\end{align*}
where $P^{A}\in\Omega^{p}\left(  \mathcal{X}\right)  $ and $Q^{B}\in\Omega
^{q}\left(  \mathcal{X}\right)  $. The commutator $\left[  P,Q\right]  $ is
defined by%
\begin{align*}
\left[  P,Q\right]   &  =P^{A}\wedge Q^{B}\left[  \mathrm{T}_{A}%
,\mathrm{T}_{B}\right]  ,\\
&  =P^{A}\wedge Q^{B}C_{AB}^{~~C}\mathrm{T}_{C}.
\end{align*}


Since $\mathrm{T}_{e}\left(  \mathcal{G}\right)  =\mathfrak{g}$, it is
interesting to define a way to map vectors between different tangent spaces.
Let $\mathcal{X}$ and $\mathcal{W}$ be two manifolds and let $f:\mathcal{X}$
$\longrightarrow\mathcal{W}$ be a map between them. We denote by $f^{\ast}$ to
the reciprocal image or \textit{pullback} induced by $f$ over a form in
$\mathcal{X}$ to a form in $\mathcal{W}$. Moreover, we denote by $f_{\ast}$ to the direct image
or \textit{pushforward} induced from a vector in $\mathcal{W}$ to a vector in
$\mathcal{X}$. In this way, given a vector $X\left(  g\right)  \in
T_{g}\left(  \mathcal{G}\right)  $, the corresponding element of the Lie
algebra $\mathrm{X}\in\mathrm{T}_{e}\left(  \mathcal{G}\right)  =\mathfrak{g}$
is given by%
\begin{equation}
\mathrm{X}=L_{g^{-1}\ast}\left(  X\left(  g\right)  \right)  .
\end{equation}
This operation induces the definition of the canonical form of a Lie group,
 the\textit{ Maurer--Cartan form} $\mathrm{\theta}\left(  g\right)  \in\Omega
^{1}\left(  \mathcal{G}\right)  \otimes\mathfrak{g}$, as the form which
satisfies%
\begin{equation}
\mathrm{\theta}\left(  g\right)  \left(  X\left(  g\right)  \right)
=\mathrm{X}.
\end{equation}

Given a matrix representation of $\mathcal{G}$, it is direct to show that the
condition%
\begin{equation*}
\mathrm{\theta}\left(  g\right)  \left(  X\left(  g\right)  \right)
=L_{g^{-1}\ast}\left(  X\left(  g\right)  \right)
\end{equation*}
implies%
\begin{equation}
\mathrm{\theta}\left(  g\right)  =g^{-1}d_{\mathcal{G}}g, \label{pr5}%
\end{equation}
where $d_{\mathcal{G}}$ is the exterior derivative over $\mathcal{G}$. Since
$\mathrm{\theta~}=\theta^{A}\mathrm{T}_{A}$, the components $\theta^{A}$ form
a dual representation of the Lie algebra and satisfy the Maurer--Cartan
structure equations%
\begin{equation}
d_{\mathcal{G}}\theta^{C}+\frac{1}{2}C_{AB}^{~~C}\theta^{A}\wedge\theta
^{B}=0.\label{pr2}%
\end{equation}
The Maurer--Cartan equations are dual to eq.$\left(  \ref{pr1}\right)  $, they
carry the same information. Thus, the dual version of the Jacobi identity is
simply the exterior derivative of eq.$\left(  \ref{pr2}\right)  $,%
\begin{equation*}
\frac{1}{2}C_{AB}^{~~C}C_{DC}^{~~E}\theta^{D}\wedge\theta^{A}\wedge\theta
^{B}=0.
\end{equation*}

\section{Connections over principal bundles}

By definition, any principal fibre bundle $\mathcal{P}$ is locally a structure
of the form $U\times\mathcal{G}$. It seems reasonable though to expect that
the tangent space associated with the fiber bundle can be decomposed in a
direct sum structure. This decomposition can be made in such a way that the
tangent space $T_{p}(\mathcal{P})$ is the direct sum of a \textit{vertical} component, tangent to
the fibre $\mathcal{G}$, and a horizontal component which is orthogonal
respect to $\mathcal{G}$. This operation is systematically implemented by
using the so called \textit{Ehresmann Connection.}

Let $T_{p}\left(  \mathcal{P}\right)  $ be the tangent space associated to the principal
bundle $\mathcal{P}$ at the point $p$, and let us decompose it as $T_{p}\left(
\mathcal{P}\right)  =V_{p}\left(  \mathcal{P}\right)  \oplus H_{p}\left(
\mathcal{P}\right)  $. Here, the vertical space $V_{p}\left(  \mathcal{P}\right)  $ corresponds to
the tangent space respect to the fibre $\mathcal{G}$ and $H_{p}\left(
\mathcal{P}\right)  ,$ the horizontal subspace, is its orthogonal complement. This motivates the following

\begin{definition}
The vertical subspace $V_{p}\left(  \mathcal{P}\right)  $ of $T_{p}\left(
\mathcal{P}\right)  $ is defined as the kernel of $\pi_{\ast}$%
\begin{equation}
V_{p}\left(  \mathcal{P}\right)  =\left\{  Y\in T_{p}\left(  \mathcal{P}%
\right)  \text{ such that }\pi_{\ast}\left(  Y\right)  =0\right\}  .
\label{pr17}%
\end{equation}

\end{definition}

In order to define the horizontal subspace $H_{p}\left(  \mathcal{P}\right)  $
in a unique way, it is necessary to define first the notion of connection over
the principal bundle:
\begin{definition}
Let $\mathrm{\omega}\in\Omega^{1}\left(  \mathcal{P}\right)  \otimes
\mathfrak{g}$ be a one form over $\mathcal{P}$ valued in the Lie algebra
$\mathfrak{g}$ satisfying the following conditions
\begin{enumerate}
\item $\mathcal{\omega}$ is continuous and smooth on $\mathcal{P},$
\item for all $Y\in V_{p}\left(  \mathcal{P}\right)  $, it holds%
\begin{equation}
\mathrm{\omega}\left(  Y\right)  =\mathrm{\theta}\left(  y_{\alpha}\left(
p\right)  \right)  \left(  y_{\alpha\ast}Y\right)  =\mathrm{Y}, \label{pr4}%
\end{equation}
\item the right action of the group is given by%
\begin{equation*}
R_{g}^{\ast}\left(  \mathrm{\omega}\left(  pg\right)  \right)  =g^{-1}%
\mathrm{\omega}\left(  p\right)  g
\end{equation*}
where $R_{g}^{\ast}$ is the pullback induced by the right action $p^{\prime
}=pg$.
\end{enumerate}
\end{definition}
The form $\mathrm{\omega}$ satisfying these properties is called
one--form \textit{connection}. From the first property one sees that
$\mathrm{\omega}$ is globally defined on $\mathcal{P}$. The second condition
implies that $\mathrm{\omega}$ associates to every vector in $V_{p}\left(
\mathcal{P}\right)  $ its corresponding element in the Lie algebra $\mathfrak{g}$ where
$y_{\alpha\ast}$ represents the pushforward $y_{\alpha\ast}:T_{p}\left(
\mathcal{P}\right)  \longrightarrow\mathcal{G}$ induced by the map $y_{\alpha
}:\mathcal{P}\longrightarrow\mathcal{G}$. Given this definition it is time to
define the horizontal subspace

\begin{definition}
The horizontal subspace it is defined as the kernel of $\mathcal{\omega}$%
\begin{equation*}
H_{p}\left(  \mathcal{P}\right)  \equiv\left\{  X\in T_{p}\left(
\mathcal{G}\right)  \text{ such that }\mathrm{\omega}\left(  X\right)
=0\right\}  .
\end{equation*}
\end{definition}

In this way, given a one--form connection $\mathrm{\omega}$, a unique
definition for $H_{p}\left(  \mathcal{P}\right)  $ is constructed. This
definition fulfils the consistency condition
\begin{equation}
H_{pg}\left(  \mathcal{P}\right)  =R_{g\ast}H_{p}\left(  \mathcal{P}\right),
\label{pr8}%
\end{equation}
so the distribution of $H_{p}\left(  \mathcal{P}\right)  $ it is invariant
under the action of $\mathcal{G}$. In fact, let $X\in H_{p}\left(
\mathcal{P}\right)  ;$ then%
\begin{equation*}
\mathrm{\omega}\left(  R_{g\ast}X\right)  =R_{g\ast}\mathrm{\omega}\left(
X\right)  =0,
\end{equation*}
and therefore $R_{g\ast}X\in H_{pg}\left(  \mathcal{P}\right)  .$

\subsection{The gauge potential}

The one--form connection $\mathrm{\omega}$ is intimately ligated with the
concept of gauge potential in the context of gauge theories.

\begin{definition}
Let $\sigma_{\alpha}:P\longrightarrow U_{\alpha}$ be a local section and
$\mathrm{\omega}$ a one--form connection over $\mathcal{P}$. Then the gauge
potential or connection is defined as
\begin{equation}
\mathcal{A}_{\alpha}=\sigma_{\alpha}^{\ast}\left(  \mathrm{\omega}\right)
\label{pr3}%
\end{equation}
where the $\ast$ denotes the pullback map which projects the connection
$\mathcal{\omega}$ to the open set $U_{\alpha}\subset\mathcal{M}$.
\end{definition}
Now, given to open sets $U_{\alpha}$ and $U_{\beta}$ with non-empty overlap
$U_{\alpha}\cap U_{\beta}\neq\varnothing$ one has two gauge connections
$\mathcal{A}_{\alpha}=\sigma_{\alpha}^{\ast}\left(  \mathrm{\omega}\right)  $
and $\mathcal{A}_{\beta}=\sigma_{\beta}^{\ast}\left(  \mathrm{\omega}\right)
$. In order to find the relation between the two gauge potentials, let us
consider a vector $X\in T_{x}\left(  U_{\alpha}\cap U_{\beta}\right)  $. The
direct image $\sigma_{\beta\ast}:T_{x}\left(  U_{\alpha}\cap U_{\beta}\right)
\longrightarrow T_{\sigma_{\beta}\left(  x\right)  }\left(  \mathcal{P}%
\right)  $ can be expressed as it follows%
\begin{align*}
\sigma_{\beta\ast}X &  =\left[  \sigma_{\alpha}\left(  x\right)  \tau
_{\alpha\beta}\left(  x\right)  \right]  _{\ast}\left(  X\right),  \\
&  =R_{\tau_{\alpha\beta\ast}}\circ\sigma_{\alpha\ast}\left(  X\right)
+\sigma_{\alpha}\left(  x\right)  _{\ast}\circ\tau_{\alpha\beta\ast}\left(
X\right).
\end{align*}
Considering the following direct images%
\begin{align*}
\tau_{\alpha\beta\ast} &  :T_{x}\left(  U_{\alpha}\cap U_{\beta}\right)
\longrightarrow T_{\tau_{\alpha\beta}\left(  x\right)  }\left(  \mathcal{G}%
\right)  ,\\
\sigma_{\alpha}\left(  x\right)  _{\ast} &  =T_{\tau_{\alpha\beta}\left(
x\right)  }\left(  \mathcal{G}\right)  \longrightarrow T_{\sigma_{\alpha
}\left(  x\right)  \tau_{\alpha\beta}\left(  x\right)  }\left(  \mathcal{P}%
\right)  ,\\
\sigma_{\alpha\ast} &  :T_{x}\left(  U_{\alpha}\cap U_{\beta}\right)
\longrightarrow T_{\sigma_{\alpha}\left(  x\right)  }\left(  \mathcal{P}%
\right)  ,\\
R_{\tau_{\alpha\beta\ast}} &  :T_{\sigma_{\alpha}\left(  x\right)  }\left(
\mathcal{P}\right)  \longrightarrow T_{\sigma_{\alpha}\left(  x\right)
\tau_{\alpha\beta}\left(  x\right)  }\left(  \mathcal{P}\right),
\end{align*}
eq.$\left(  \ref{pr3}\right)  $ reads%
\begin{align*}
\mathcal{A}_{\beta}\left(  X\right)   &  =\sigma_{\beta}^{\ast}\mathrm{\omega
}\left(  X\right), \\
&  =\mathrm{\omega}\left(  \sigma_{\beta\ast}X\right), \\
&  =\mathrm{\omega}\left(  R_{\tau_{\alpha\beta\ast}}\circ\sigma_{\alpha\ast
}\left(  X\right)  \right)  +\mathrm{\omega}\left(  \sigma_{\alpha}\left(
x\right)  _{\ast}\circ\tau_{\alpha\beta\ast}\left(  X\right)  \right).
\end{align*}
Using eq.$\left(  \ref{pr4}\right)  $, we find%
\begin{equation*}
\mathrm{\omega}\left(  \sigma_{\alpha}\left(  x\right)  _{\ast}\circ
\tau_{\alpha\beta\ast}\left(  X\right)  \right)  =\mathrm{\theta}\left(
\tau_{\alpha\beta}\right)  \left(  \tau_{\alpha\beta\ast}\left(  X\right)
\right)  ,
\end{equation*}
and using eq.$\left(  \ref{pr5}\right)  $%
\begin{align*}
\mathcal{A}_{\beta}\left(  X\right)   &  =\sigma_{\alpha}^{\ast}\left(
\tau_{\alpha\beta}^{-1}\mathcal{\omega}\tau_{\alpha\beta}\right)  \left(
X\right)  +\left(  \tau_{\alpha\beta}^{-1}d_{\mathcal{G}}\tau_{\alpha\beta
}\right)  \left(  \tau_{\alpha\beta\ast}X\right)  ,\\
&  =\tau_{\alpha\beta}^{-1}\sigma_{\alpha}^{\ast}\left(  \mathcal{\omega
}\right)  \tau_{\alpha\beta}\left(  X\right)  +\tau_{\alpha\beta}^{\ast
}\left(  \tau_{\alpha\beta}^{-1}d_{\mathcal{G}}\tau_{\alpha\beta}\right)
\left(  X\right)  ,\\
&  =\left(  \tau_{\alpha\beta}^{-1}\mathcal{A}_{\alpha}\tau_{\alpha\beta}%
+\tau_{\alpha\beta}^{-1}d_{\mathcal{M}}\tau_{\alpha\beta}\right)  \left(
X\right)  ,
\end{align*}
we finally arrive to%
\begin{equation}
\mathcal{A}_{\beta}=\tau_{\alpha\beta}^{-1}\mathcal{A}_{\alpha}\tau
_{\alpha\beta}+\tau_{\alpha\beta}^{-1}d_{\mathcal{M}}\tau_{\alpha\beta}.
\label{pr6}%
\end{equation}

The relation between the gauge connections eq.$\left(  \ref{pr6}\right)  $ is
what in physics it is known as \textit{gauge transformations}. If the
principal $\mathcal{P}$ bundle is not trivial, there always exists
$\tau_{\alpha\beta}\left(  x\right)  \in\mathcal{G}$ such that the connection
$\mathcal{A}_{\alpha}$ over $U_{\alpha}$ and the connection $\mathcal{A}%
_{\beta}$ over $U_{\beta}$ are related by eq.$\left(  \ref{pr6}\right)  $ over
$U_{\alpha}\cap U_{\beta}$. In the future we write $g=\tau_{\alpha\beta
}\left(  x\right)  $ and $d=d_{\mathcal{M}}$ to avoid overload notation. In
this way eq.$\left(  \ref{pr6}\right)  $ reads%
\begin{equation}
\mathcal{A\longrightarrow A}^{\prime}=g^{-1}\mathcal{A}g+g^{-1}dg. \label{pr7}%
\end{equation}

\subsection{Covariant derivative and curvature}

The definition of connection over $\mathcal{P}$ implies that $\mathrm{\omega}$
projects any vector in $T_{p}\left(  \mathcal{P}\right)  $ only to its vertical
component. It seems natural then to consider a $b$--form $\mathrm{B}\in$
$\Omega^{b}\left(  \mathcal{P}\right)  \otimes\mathfrak{g}$ which projects vectors in $T_{p}\left(  \mathcal{P}\right)  $ to the
horizontal component $H_{p}\left(  \mathcal{P}\right)  $.
Let $h:T_{p}\left(  \mathcal{P}\right)  \longrightarrow H_{p}\left(
\mathcal{P}\right)  $ be a map such that to every vector $Z\in T_{p}\left(
\mathcal{P}\right)  $ it associate its projection over the horizontal subspace
$Z^{h}=h\left(  Z\right)  $. With the help of this map $h$, tensor and pseudo
tensorial forms will be defined.
\begin{definition}
a $b$--form $\mathrm{B~}$over $\mathcal{P}$ is called pseudotensorial when it
satisfies
\begin{equation*}
R_{g}^{\ast}\left(  \mathrm{B}\left(  pg\right)  \right)  =g^{-1}\mathrm{B}g,
\end{equation*}
where $R_{g}^{\ast}$ is the reciprocal image induced by the right action
$p^{\prime}=pg$. The form $B$ is called tensorial if
\begin{equation*}
\mathrm{B}\left(  Z_{1},\ldots,Z_{b}\right)  =\mathrm{B}\left(  Z_{1}%
^{h},\ldots,Z_{b}^{h}\right)  ,
\end{equation*}
where $Z_{i}^{h}=h\left(  Z_{i}\right)  $, $i=1,\ldots,b$.
\end{definition}

The name \textit{tensorial form} has it origin in the following theorem

\begin{theorem}
Let $\mathrm{B}$ be a tensorial form over $\mathcal{P}$. Then, on the
intersection $U_{\alpha}\cap U_{\beta}\neq\varnothing$ it follows%
\begin{equation*}
\mathcal{B}_{\beta}=\tau_{\alpha\beta}^{-1}\mathcal{B}_{\alpha}\tau
_{\alpha\beta},%
\end{equation*}
where the $b$--form $\mathcal{B}\in\mathcal{M}$ corresponds to $\mathcal{B}%
_{\alpha}=\sigma_{\alpha}^{\ast}\mathrm{B}$.

\begin{proof}
In fact, we have%
\begin{align*}
R_{g}^{\ast}\mathrm{B}\left(  p\right)  \left(  Z_{1}\left(  p\right)
,\ldots,Z_{b}\left(  p\right)  \right)   &  =R_{g}^{\ast}\mathrm{B}\left(
p\right)  \left(  Z_{1}^{h}\left(  p\right)  ,\ldots,Z_{b}^{h}\left(
p\right)  \right)  ,\\
&  =\mathrm{B}\left(  pg\right)  \left(  R_{\ast g}Z_{1}^{h}\left(  p\right)
,\ldots,R_{\ast g}Z_{b}^{h}\left(  p\right)  \right)  .
\end{align*}
Using eq.$\left(  \ref{pr8}\right)  $
\begin{align*}
R_{g}^{\ast}\mathrm{B}\left(  p\right)  \left(  Z_{1}\left(  p\right)
,\ldots,Z_{b}\left(  p\right)  \right)   &  =\mathrm{B}\left(  pg\right)
\left(  Z_{1}^{h}\left(  pg\right)  ,\ldots,Z_{b}^{h}\left(  pg\right)
\right) \\
&  =\mathrm{B}\left(  pg\right)  \left(  Z_{1}\left(  pg\right)  ,\ldots
,Z_{b}\left(  pg\right)  \right)
\end{align*}
Thus, when $\mathrm{B}$ is tensorial,%
\begin{equation}
R_{g}^{\ast}\mathrm{B}\left(  p\right)  \left(  Z_{1}\left(  p\right)
,\ldots,Z_{b}\left(  p\right)  \right)  =\mathrm{B}\left(  pg\right)  \left(
Z_{1}\left(  pg\right)  ,\ldots,Z_{b}\left(  pg\right)  \right)  . \label{pr9}%
\end{equation}
Repeating the procedure used to deduce the gauge transformation eq.$\left(
\ref{pr7}\right)  $ one concludes that, in the intersection $U_{\alpha}\cap
U_{\beta},$%
\begin{equation}
\mathcal{B}_{\beta}=\tau_{\alpha\beta}^{-1}\mathcal{B}_{\alpha}\tau
_{\alpha\beta}. \label{pr10}%
\end{equation}

\end{proof}
\end{theorem}

This theorem lead us naturally to another definition; the definition of the
exterior covariant derivative operator $\mathcal{D}$

\begin{definition}
Let $\mathrm{B}$ be a pseudotensorial form over $\mathcal{P}$. Then, the
exterior covariant derivative is defined as%
\begin{equation*}
\mathcal{D}\mathrm{B}=d_{\mathcal{P}}\mathrm{B}\circ h,
\end{equation*}
where $d_{\mathcal{P}}$ denotes the exterior derivative in $\mathcal{P}$.
Using the same arguments that we used to show eq.$\left(  \ref{pr9}\right)  $,
it is possible to show that when $\mathrm{B}$ is a pseudotensorial form, then
$\mathcal{D}\mathrm{B}$ is a $\left(  b+1\right)  $--tensorial form.
\end{definition}

Since the connection $\mathrm{\omega}$ is pseudotensorial, it is possible to
define the tensorial two--form $\mathrm{F}$ as
\begin{equation*}
\mathrm{F}=\mathcal{D}\mathrm{\omega},
\end{equation*}
which is called the \textit{curvature} of the principal bundle $\mathcal{P}$. Also, it
is possible to show (see Theorem 2.13 Ref.\cite{deAz95})  directly that%
\begin{equation*}
\mathrm{F}=d_{\mathcal{P}}\mathrm{\omega}+\frac{1}{2}\left[  \mathrm{\omega
},\mathrm{\omega}\right]
\end{equation*}
Given the curvature $\mathrm{F}$ over the principal bundle $\mathcal{P}$, it
is direct to define the gauge curvature or \textit{field strength} over an open
set $U_{\alpha}$ as $\mathcal{F}_{\alpha}=\sigma_{\alpha}^{\ast
}\mathrm{F}$. In terms of eq.$\left(  \ref{pr3}\right)  $, the curvature
$\mathcal{F}_{\alpha}$ corresponds to%
\[
\mathcal{F}_{\alpha}=d_{\mathcal{M}}\mathcal{A}_{\alpha}+\mathcal{A}_{\alpha
}\wedge\mathcal{A}_{\alpha}.
\]
Now, $\mathrm{F}$ is tensorial so it satisfy eq.$\left(  \ref{pr10}\right)
$%
\begin{equation*}
\mathcal{F}_{\beta}=\tau_{\alpha\beta}^{-1}\mathcal{F}_{\alpha}\tau
_{\alpha\beta},%
\end{equation*}
and it is direct to verify the consistency with eq.$\left(  \ref{pr6}\right)
$.

On a tensorial $b$--form $\mathrm{B}\in\Omega^{b}\left(  \mathcal{P}\right)
\otimes\mathfrak{g}$, it is possible to show (see p.$94$ Ref.\cite{deAz95}) that its covariant
derivative $\mathcal{D}\mathrm{B}$ is given by%
\begin{equation*}
\mathcal{D}\mathrm{B}=d_{\mathcal{P}}\mathrm{B}+\left[  \mathrm{\omega
},\mathrm{B}\right].
\end{equation*}
Moreover, the derivative operator $\mathcal{D}$ satisfy the Bianchi Identities%
\begin{align}
\mathcal{DD}\mathrm{B}  &  =\left[  \mathrm{F},\mathrm{B}\right]  ,\nonumber\\
\mathcal{D}\mathrm{F}  &  =0. \label{pr19}%
\end{align}

In the base space $\mathcal{M}$, the covariant derivative is obtained by the projection
\begin{align}
D_{\alpha}\mathcal{B}_{\alpha}  &  =\sigma_{\alpha}^{\ast}\left(
\mathcal{D}\mathrm{B}\right)  ,\nonumber\\
&  =d_{\mathcal{M}}\mathcal{B}_{\alpha}+\left[  \mathcal{A}_{\alpha
},\mathcal{B}_{\alpha}\right]  , \label{pr12}%
\end{align}
and the Bianchi identities are given by%
\begin{align*}
D_{\alpha}D_{\alpha}\mathcal{B}_{\alpha}  &  =\left[  \mathcal{F}_{\alpha
},\mathcal{B}_{\alpha}\right]  ,\\
D_{\alpha}\mathcal{F}  &  =0.
\end{align*}
Note that, by definition, $\mathcal{D}\mathrm{B}$ is tensorial and therefore
it satisfies
\begin{equation*}
D_{\beta}\mathcal{B}_{\beta}=\tau_{\alpha\beta}^{-1}D_{\alpha}\mathcal{B}%
_{\alpha}\tau_{\alpha\beta},%
\end{equation*}
and again, this is consistent with the gauge transformation eq.$\left(
\ref{pr6}\right)  $.





\section{Transgression forms and the Chern class}
Given the notion of principal bundle $\mathcal{P}$ and connection $\mathrm{\omega}$, it is interesting to study the existence of characteristic quantities defined over $\mathcal{P}$. In principle, this quantities are defined in terms of the connection $\mathrm{\omega}$. However, it turns out that they are completely independent of the choice of $\mathrm{\omega}$. Thus, these quantities define \textit{topological invariants} which measure the obstruction of the bundle $\mathcal{P}$ to be trivial. 

In the following, we first introduce some preliminary definitions and then we will use the Chern--Weil theorem to define the Transgression form and the Chern Class.

\subsection{Invariant Polynomial}

\begin{definition}
An invariant polynomial of degree $n$, is a $n-$linear map%
\begin{equation*}
\left\vert \ldots\right\vert :\underset{n\text{ times}}{\underbrace
{\mathfrak{g\times}\ldots\times\mathfrak{g}}}\longrightarrow%
\mathbb{R}
\end{equation*}
which satisfy the condition%
\begin{equation}
\left\vert \left(  g^{-1}\mathrm{Z}_{1}g\right)  \wedge\ldots\wedge\left(
g_{n}^{-1}\mathrm{Z}g\right)  \right\vert =\left\vert \mathrm{Z}_{1}%
\wedge\ldots\wedge\mathrm{Z}_{n}\right\vert \label{pr11}%
\end{equation}
where $\mathrm{Z}\in\Omega^{z_{i}}\otimes\mathfrak{g}$, $i=1,\ldots,n$ and
$g=exp(\lambda^A \mathrm{T}_A)\in\mathcal{G}$. When the extra condition
\begin{equation*}
\left\vert \mathrm{Z}_{1}\wedge\ldots\wedge\mathrm{Z}_{i}\wedge\ldots
\wedge\mathrm{Z}_{j}\wedge\ldots\wedge\mathrm{Z}_{n}\right\vert =\left(
-1\right)  ^{z_{i}z_{j}}\left\vert \mathrm{Z}_{1}\wedge\ldots\wedge
\mathrm{Z}_{j}\wedge\ldots\wedge\mathrm{Z}_{i}\wedge\ldots\wedge\mathrm{Z}%
_{n}\right\vert
\end{equation*}
is satisfied for all $\mathrm{Z}_{i},\mathrm{Z}_{j}$, we say that the
invariant polynomial is symmetric and we denote it by $\left\langle
\ldots\right\rangle $.
\end{definition}

Since $\mathrm{Z}=Z^{A}\mathrm{T}_{A}$, it is possible to write
\begin{equation*}
\left\langle \mathrm{Z}_{1}\wedge\ldots\wedge\mathrm{Z}_{n}\right\rangle
=Z_{1}^{A_{1}}\wedge\ldots\wedge Z_{n}^{A_{n}}\left\langle \mathrm{T}_{A_{1}%
}\ldots\mathrm{T}_{A_{n}}\right\rangle,
\end{equation*}
where $\left\langle \mathrm{T}_{A_{1}}\ldots\mathrm{T}_{A_{n}}\right\rangle $
it is called a symmetric invariant tensor. The invariance condition
eq.$\left(  \ref{pr11}\right)  $ can be written in different ways. In fact, if
we consider an element $g=\exp\left(  \lambda^{A}\mathrm{T}_{A}\right)
\in\mathcal{G}$ infinitesimally close to the identity, the invariant condition
takes the form%
\begin{equation*}
\left\langle \left[  \lambda,\mathrm{Z}_{1}\right]  \wedge\mathrm{Z}_{2}%
\wedge\ldots\wedge\mathrm{Z}_{n}\right\rangle +\ldots+\left\langle
\mathrm{Z}_{1}\wedge\ldots\wedge\mathrm{Z}_{n-1}\wedge\left[  \lambda
,\mathrm{Z}_{n}\right]  \right\rangle =0
\end{equation*}
where $\lambda=\lambda^{A}\mathrm{T}_{A}$. Identifying $\lambda$ with the
one--form connection $\mathcal{A}$ and recalling the definition of covariant
derivative eq.$\left(  \ref{pr12}\right)  $, the invariance conditions is
given by%
\begin{equation}
\left\langle D\left(  \mathrm{Z}_{1}\wedge\ldots\wedge\mathrm{Z}_{n}\right)
\right\rangle =d\left\langle \mathrm{Z}_{1}\wedge\ldots\wedge\mathrm{Z}%
_{n}\right\rangle .\label{pr21}%
\end{equation}
All this expression for the invariance condition will be used through this
thesis depending on the context.

\subsection{Projection of differential forms}

So far, we have defined differential forms over the base space $\mathcal{M}$
starting from differential forms defined over the principal bundle
$\mathcal{P}$. In order to do so, we used the reciprocal image induced by the
local sections $\sigma_{\alpha}:U_{\alpha}\subset\mathcal{M\rightarrow P}%
$. A natural question is if one can do the opposite, i.e, defining a form in
$\mathcal{P}$ starting from a form defined over $\mathcal{M}$. This is
possible by using the pullback of the projection map $\pi
:\mathcal{P\rightarrow M}$.

Given a $p-$form $\mathcal{B}$ over $\mathcal{M}$ it is possible to construct
a $p-$form $\mathrm{B}$ over $\mathcal{P}$ as%
\begin{equation*}
\mathrm{B}=\pi^{\ast}\mathcal{B}.%
\end{equation*}
Now, given two points of the same fiber $p$ and $p^{\prime}=pg$ and a $p-$form
$\mathrm{B}$, in general it is true that $\mathrm{B}\left(  p\right)  $ and
$\mathrm{B}\left(  pg\right)  $ will correspond to the pullback of different
$p-$forms over $\mathcal{M}$,%
\begin{align*}
\mathrm{B}(p)   &  =\pi^{\ast}\mathcal{B}(x)  \\
\mathrm{B}(pg)   &  =\pi^{\ast}\mathcal{B}^{\prime}(x)
\end{align*}
with $\mathcal{B}(x)  \neq\mathcal{B}^{\prime}(x)  $
in general. When the $p-$form $\mathrm{B}$ along the fiber $\pi^{-1}(
x)  $ corresponds to the pullback of a unique $p-$form $\mathcal{B}%
(x)  $, we say that \textrm{B} is projectable to $\mathcal{B}%
(x)  $. Let us precise the notion of projectable differential
form in terms of the following
\begin{theorem}
Let $\mathrm{B}$ be a $p-$form over $\mathcal{P}$ satisfying
\begin{enumerate}
\item $\mathrm{B}$ is right invariant under the action of $\mathcal{G}$,%
\begin{equation}
R_{g}^{\ast}\mathrm{B}=\mathrm{B} \label{pr14}%
\end{equation}
\item $\mathrm{B}$ acts on $T_{p}\left(  \mathcal{P}\right)  $ in such a way
that%
\begin{equation}
\mathrm{B}\left(  X_{1}\ldots X_{n}\right)  =\mathrm{B}\left(  X_{1}^{h}\ldots
X_{n}^{h}\right)  \label{pr13}%
\end{equation}
then, there exist a unique $p-$form $\mathcal{B}(x)  $ defined
over $\mathcal{M}$ such that $\mathrm{B}=\pi^{\ast}\mathcal{B}$ and therefore
$\mathrm{B}$ is projectable.
\end{enumerate}
\end{theorem}

\begin{proof}
Let $X_{i}\left(  p\right)  \in T_{p}\left(  \mathcal{P}\right)  $ with
$i=1,\ldots,q$. Consider the pushforward induced by the projection map $\pi$%
\begin{align*}
\pi_{\ast} &  :T_{p}\left(  \mathcal{P}\right)  \longrightarrow T_{x}\left(
\mathcal{M}\right)  .\\
&  :X_{i}\left(  p\right)  \longrightarrow Y_{i}\left(  x\right)  =\pi_{\ast
}X_{i}(p)
\end{align*}
Let $\mathcal{B}(x)  $ be a $q-$form such that%
\begin{equation*}
\mathrm{B}\left(  p\right)  =\pi^{\ast}\mathcal{B}\left(  x\right)  .
\end{equation*}
Then, we have
\begin{align*}
\mathcal{B}\left(  x\right)  \left(  Y_{1}\left(  x\right)  ,\ldots
,Y_{q}\left(  x\right)  \right)   &  =\mathcal{B}\left(  x\right)  \left(
\pi_{\ast}X_{1}\left(  p\right)  ,\ldots,\pi_{\ast}X_{q}\left(  p\right)
\right)  ,\\
&  =\pi^{\ast}\mathcal{B}\left(  x\right)  \left(  X_{1}\left(  p\right)
,\ldots,X_{q}\left(  p\right)  \right)  ,\\
&  =\mathrm{B}\left(  p\right)  \left(  X_{1}\left(  p\right)  ,\ldots
,X_{q}\left(  p\right)  \right)  ,
\end{align*}
and using eq.$\left(  \ref{pr13}\right)  $,%
\begin{equation}
\pi^{\ast}\mathcal{B}\left(  x\right)  \left(  X_{1}\left(  p\right)
,\ldots,X_{q}\left(  p\right)  \right)  =\mathrm{B}\left(  p\right)  \left(
X_{1}^{h}\left(  p\right)  ,\ldots,X_{q}^{h}\left(  p\right)  \right)
.\label{pr15}%
\end{equation}
Now, using eq.$\left(  \ref{pr8}\right)  $%
\begin{align*}
\mathrm{B}\left(  pg\right)  \left(  X_{1}^{h}\left(  pg\right)  ,\ldots
,X_{q}^{h}\left(  pg\right)  \right)   &  =\mathrm{B}\left(  pg\right)
\left(  R_{g\ast}X_{1}^{h}\left(  p\right)  ,\ldots,R_{g\ast}X_{q}^{h}\left(
p\right)  \right)  ,\\
&  =R_{g}^{\ast}\mathrm{B}\left(  p\right)  \left(  X_{1}^{h}\left(  p\right)
,\ldots,X_{q}^{h}\left(  p\right)  \right)  ,
\end{align*}
Finally, using eq.$\left(  \ref{pr14}\right)  $ we have%
\begin{equation}
\mathrm{B}\left(  pg\right)  \left(  X_{1}^{h}\left(  pg\right)  ,\ldots
,X_{q}^{h}\left(  pg\right)  \right)  =\mathrm{B}\left(  p\right)  \left(
X_{1}^{h}\left(  p\right)  ,\ldots,X_{q}^{h}\left(  p\right)  \right),
\label{pr16}%
\end{equation}
and comparing eq.$\left(  \ref{pr15}\right)  $ with eq.$\left(  \ref{pr16}%
\right)  $ one sees that $\mathrm{B}\left(  pg\right)  $ and $\mathrm{B}\left(
p\right)  $ corresponds to the pullback of the same form $\mathcal{B}(x)  $%
\begin{equation*}
\mathrm{B}\left(  pg\right)  \left(  X_{1}^{h}\left(  pg\right)  ,\ldots
,X_{q}^{h}\left(  pg\right)  \right)  =\pi^{\ast}\mathcal{B}\left(  x\right)
\left(  X_{1}\left(  p\right)  ,\ldots,X_{q}\left(  p\right)  \right).
\end{equation*}
Thus, the form $\mathcal{B}\left(  x\right)  $ is the projection of
$\mathrm{B}$.
\end{proof}

The important thing about the projection operation is that given a smooth
$p-$form $\mathrm{B}$ defined over $\mathcal{P}$, its projection
$\mathcal{B}\left(  x\right)  $ gives a $p-$form \textit{globally} defined
over the base space $\mathcal{M}$. This is in contrast with the construction
of differential forms by using the pullback induced by local sections
$\sigma_{\alpha}$; in the sense that given a globally defined $p-$form over
$\mathcal{P}$, in general it is only possible to obtain $p-$forms locally
defined in an open set $U_{\alpha}\subset\mathcal{M}$.

However, it is possible to find relations between both procedures. In order to
do so, it is necessary to observe that given an arbitrary local section
$\sigma_{\alpha}$, it is always possible to find an element $g_{\alpha}%
\in\mathcal{G}$ such that%
\[
\sigma_{\alpha}\circ\pi=g_{\alpha}.
\]
Now, if $\mathrm{B}$ is projectable,
\begin{align*}
\mathrm{B} &  =R_{g_{\alpha}}^{\ast}\mathrm{B},\\
&  =R_{\sigma_{\alpha}\circ\pi}^{\ast}\mathrm{B},\\
&  =\pi^{\ast}\sigma_{\alpha}^{\ast}\mathrm{B},%
\end{align*}
and writing $\mathcal{B}_{\alpha}\mathcal{=\sigma}_{\alpha}^{\ast}\mathrm{B}$,
we have%
\begin{equation}
\mathrm{B}=\pi^{\ast}\mathcal{B}_{\alpha}.\label{pr20}%
\end{equation}
Since $\mathrm{B}$ is projectable, its projection $\mathcal{B}$ is such that
$\mathrm{B}=\pi^{\ast}\mathcal{B}$ is unique. This means that in the non-empty 
overlap $U_{\alpha}\cap U_{\beta}$, the forms $\mathcal{B}$ are equivalent
\begin{equation*}
\mathcal{B}_{\alpha}=\mathcal{B}_{\beta}=\mathcal{B}%
\end{equation*}
and globally defined over $\mathcal{M}$.

An important property about the projection operation is its relation with the
covariant derivative operator $\mathcal{D}$ over the principal bundle $\mathcal{P}$.

\begin{theorem}
If $\mathrm{B}$ is projectable, then%
\begin{equation}
\mathcal{D}\mathrm{B}=d_{\mathcal{P}}\mathrm{B}\text{.} \label{pr18}%
\end{equation}

\end{theorem}

\begin{proof}
In fact,
\begin{align*}
d_{\mathcal{P}}\mathrm{B}\left(  X_{1},\ldots,X_{p}\right)   &
=d_{\mathcal{P}}\pi^{\ast}\mathcal{B}\left(  X_{1},\ldots,X_{p}\right)  ,\\
&  =\pi^{\ast}\left(  d_{\mathcal{M}}\mathcal{B}\right)  \left(  X_{1}%
,\ldots,X_{p}\right)  ,\\
&  =d_{\mathcal{M}}\mathcal{B}\left(  \pi_{\ast}X_{1},\ldots,\pi_{\ast}%
X_{p}\right)  ,
\end{align*}
By definition of vertical subspace, we have $\pi_{\ast}X_{i}=\pi_{\ast}X_{i}^{h}$
$\left[  \text{see\thinspace eq.}\left(  \ref{pr17}\right)  \right].  $ Thus,%
\begin{align*}
d_{\mathcal{P}}\mathrm{B}\left(  X_{1},\ldots,X_{p}\right)   &
=d_{\mathcal{M}}\mathcal{B}\left(  \pi_{\ast}X_{1}^{h},\ldots,\pi_{\ast}%
X_{p}^{h}\right)  ,\\
&  =\pi^{\ast}\left(  d_{\mathcal{M}}\mathcal{B}\right)  \left(  X_{1}%
^{h},\ldots,X_{p}^{h}\right)  ,\\
&  =d_{\mathcal{P}}\pi^{\ast}\mathcal{B}\left(  X_{1}^{h},\ldots,X_{p}%
^{h}\right)  ,\\
&  =d_{\mathcal{P}}\mathrm{B}\left(  X_{1}^{h},\ldots,X_{p}^{h}\right)  ,\\
&  =d_{\mathcal{P}}\mathrm{B}\circ h\left(  X_{1},\ldots,X_{p}\right)  ,\\
&  =\mathcal{D}\mathrm{B}\left(  X_{1},\ldots,X_{p}\right)  .
\end{align*}
and therefore%
\begin{equation*}
d_{\mathcal{P}}\mathrm{B}=\mathcal{D}\mathrm{B.}%
\end{equation*}

\end{proof}

\subsection{Chern--Weil Theorem}

\begin{theorem}
Let $\mathcal{P}\left(  \mathcal{M},\mathcal{G}\right)  $ be a principal
bundle with base space $\mathcal{M}$ endowed with a one--form connection $\mathrm{\omega
}\in\Omega^{1}\left(  \mathcal{P}\right)  \otimes\mathfrak{g}$. Let $\mathrm{F}\in\Omega^{2}\left(  \mathcal{P}\right)\otimes\mathfrak{g}$ be its
corresponding curvature, where $\mathfrak{g}$ the Lie algebra associated to the
structure group $\mathcal{G}$. Let $\left\langle \mathrm{T}_{A_{1}}%
\ldots\mathrm{T}_{A_{n+1}}\right\rangle $ be a symmetric invariant tensor of rank
$n+1$, and let $\left\langle \mathrm{F}^{n+1}\right\rangle $ be a $\left(
2n+2\right)-$form
\begin{equation*}
\left\langle \mathrm{F}^{n+1}\right\rangle =\underset{n+1\text{ times}%
}{\underbrace{\left\langle \mathrm{F}\wedge\ldots\wedge\mathrm{F}\right\rangle
}}.
\end{equation*}
Then,
\begin{enumerate}
\item $\left\langle \mathrm{F}^{n+1}\right\rangle $ is a closed form,
$d_{\mathcal{P}}\left\langle \mathrm{F}^{n+1}\right\rangle =0$ and projectable%
\begin{equation*}
\left\langle \mathrm{F}^{n+1}\right\rangle =\pi^{\ast}\left\langle
\mathcal{F}^{n+1}\right\rangle ,
\end{equation*}
with $\left\langle \mathcal{F}^{n+1}\right\rangle $ closed,  $d_{\mathcal{M}%
}\left\langle \mathcal{F}^{n+1}\right\rangle =0$.
\item Given two connections $\mathrm{\omega}$ and $\mathrm{\bar{\omega}}$ over
$\mathcal{P}$ and they respective curvatures $\mathrm{F}$ and $\mathrm{\bar{F}%
}$, the difference $\left\langle \mathrm{F}^{n+1}\right\rangle -\left\langle
\mathrm{\bar{F}}^{n+1}\right\rangle $ is an exact form and projectable.
\end{enumerate}
\end{theorem}

\begin{proof}
$\left\langle \mathrm{F}^{n+1}\right\rangle $ is projectable since it is
invariant under the right action $R_{g}^{\ast}$ of the group. In fact, given
that $\mathrm{F}$ is tensorial, we have%
\begin{equation*}
R_{g}^{\ast}\mathrm{F}=g^{-1}\mathrm{F}g,
\end{equation*}
and due to $\left\langle \mathrm{F}^{n+1}\right\rangle $ is an invariant
polynomial, it follows%
\begin{equation*}
R_{g}^{\ast}\left\langle \mathrm{F}^{n+1}\right\rangle =\left\langle
\mathrm{F}^{n+1}\right\rangle .
\end{equation*}
On the other hand, since $\mathrm{F}$ is tensorial, $\mathrm{F}\left(
X_{1},X_{2}\right)  =\mathrm{F}\left(  X_{1}^{h},X_{2}^{h}\right)  $ and
therefore%
\begin{equation*}
\left\langle \mathrm{F}^{n+1}\right\rangle \left(  X_{1},\ldots,X_{2n+2}%
\right)  =\left\langle \mathrm{F}^{n+1}\right\rangle \left(  X_{1}^{h}%
,\ldots,X_{2n+2}^{h}\right)  .
\end{equation*}
Thus, since $\left\langle \mathrm{F}^{n+1}\right\rangle $ is projectable it
fulfils eq.$\left(  \ref{pr18}\right)  $%
\begin{equation*}
d_{\mathcal{P}}\left\langle \mathrm{F}^{n+1}\right\rangle =\mathcal{D}%
\left\langle \mathrm{F}^{n+1}\right\rangle ,
\end{equation*}
and using the Bianchi identity eq.$\left(  \ref{pr19}\right)  $ we see that
$\left\langle \mathrm{F}^{n+1}\right\rangle $ is a closed form%
\begin{equation*}
d_{\mathcal{P}}\left\langle \mathrm{F}^{n+1}\right\rangle =0.
\end{equation*}
Using eq.$\left(  \ref{pr20}\right)  $ we have that the polynomial
\begin{equation*}
\left\langle \mathcal{F}_{\alpha}^{n+1}\right\rangle =\sigma_{\alpha}^{\ast
}\left\langle \mathrm{F}^{n+1}\right\rangle
\end{equation*}
corresponds to the projection of $\left\langle \mathrm{F}^{n+1}\right\rangle $
over $\mathcal{M}$ and therefore $\left\langle \mathcal{F}_{\alpha}%
^{n+1}\right\rangle $ is globally defined. In order to show that $\left\langle
\mathcal{F}_{\alpha}^{n+1}\right\rangle $ is closed, consider the Bianchi
identity%
\begin{equation*}
D_{\alpha}\left\langle \mathcal{F}_{\alpha}^{n+1}\right\rangle =0.
\end{equation*}
Making use of the invariance property eq.$\left(  \ref{pr21}\right)  $ we find%
\begin{equation*}
d_{\mathcal{M}}\left\langle \mathcal{F}_{\alpha}^{n+1}\right\rangle =0.
\end{equation*}
The quantity $\left\langle \mathcal{F}_{\alpha}^{n+1}\right\rangle ,$ with a
given normalization factor, corresponds to the $\left(  n+1\right)  $
\textit{Chern-class}%
\begin{equation*}
\mathsf{ch}_{n+1}\left(  \mathcal{F}\right)  =\frac{1}{\left(  n+1\right)
!}\left(  \frac{i}{2\pi}\right)  ^{n+1}\left\langle \mathcal{F}^{n+1}%
\right\rangle .
\end{equation*}

\end{proof}

\begin{proof}
Consider two one--form connections $\mathrm{\omega}$ and $\mathrm{\bar{\omega
}}$. The difference
\begin{equation*}
\mathrm{O}=\mathrm{\omega}-\mathrm{\bar{\omega}}%
\end{equation*}
is tensorial because given a vertical vector $Y\in V_{p}\left(  \mathcal{P}\right)  $, then%
\begin{equation*}
\mathrm{O}\left(  Y\right)  =\mathrm{Y}-\mathrm{Y}=0.
\end{equation*}
Using these two connections, it is possible to define a third interpolating connection $\mathrm{\omega}_t$ as%
\begin{equation}
\mathrm{\omega}_{t}=\mathrm{\bar{\omega}}+t\mathrm{O}\label{pr24}%
\end{equation}
where $t\in\left[  0,1\right]  $, and its corresponding curvature
\begin{align}
\mathrm{F}_{t} &  =\mathcal{D}\mathrm{\omega}_{t},\nonumber\\
&  =d_{\mathcal{P}}\mathrm{\omega}_{t}+\mathrm{\omega}_{t}\wedge
\mathrm{\omega}_{t},\nonumber\\
&  =\mathrm{\bar{F}}+t\mathcal{\bar{D}}\mathrm{O}+t^{2}\mathrm{O}%
\wedge\mathrm{O},\label{pr25}%
\end{align}
where $\mathcal{\bar{D}}\mathrm{O=}d_{\mathcal{P}}\mathrm{O}+\left[
\mathrm{\bar{\omega}},\mathrm{O}\right]  $. Now, the derivative respect to $t$
of $\mathrm{F}_{t}$ is given by%
\begin{align}
\frac{d\mathrm{F}_{t}}{dt} &  =\mathcal{\bar{D}}\mathrm{O}+t\left[
\mathrm{O},\mathrm{O}\right],  \nonumber\\
&  =\mathcal{D}_{t}\mathrm{O},\label{pr22}%
\end{align}
where%
\begin{equation*}
\mathcal{D}_{t}\mathrm{O}=d_{\mathcal{P}}\mathrm{O+}\left[  \mathrm{\omega
}_{t},\mathrm{O}\right]  .
\end{equation*}
Since $\left.  \mathrm{F}_{t}\right\vert _{t=0}=\mathrm{\bar{F}}$ and $\left.
\mathrm{F}_{t}\right\vert _{t=1}=\mathrm{F}$, it is possible to write the
difference $ \left\langle \mathrm{F}^{n+1}\right\rangle -\left\langle \mathrm{\bar{F}%
}^{n+1}\right\rangle$ as
\begin{equation*}
\left\langle \mathrm{F}^{n+1}\right\rangle -\left\langle \mathrm{\bar{F}%
}^{n+1}\right\rangle =\int_{0}^{1}dt\frac{d}{dt}\left\langle \mathrm{F}%
_{t}^{n+1}\right\rangle .
\end{equation*}
The polynomial $\left\langle \mathrm{F}_{t}^{n+1}\right\rangle $ is a $\left(  2n+2\right)-$form and symmetric. This allow us to write%
\begin{equation*}
\left\langle \mathrm{F}^{n+1}\right\rangle -\left\langle \mathrm{\bar{F}%
}^{n+1}\right\rangle =\left(  n+1\right)  \int_{0}^{1}dt\left\langle
\frac{d\mathrm{F}_{t}}{dt}\wedge\mathrm{F}_{t}^{n}\right\rangle ,
\end{equation*}
inserting eq.$\left(  \ref{pr22}\right)  $, we get%
\begin{align*}
\left\langle \mathrm{F}^{n+1}\right\rangle -\left\langle \mathrm{\bar{F}%
}^{n+1}\right\rangle  &  =\left(  n+1\right)  \int_{0}^{1}dt\left\langle
\mathcal{D}_{t}\mathrm{O}\wedge\mathrm{F}_{t}^{n}\right\rangle ,\\
&  =\left(  n+1\right)  \int_{0}^{1}dt\mathcal{D}_{t}\left\langle
\mathrm{O}\wedge\mathrm{F}_{t}^{n}\right\rangle.
\end{align*}
where we have used the Bianchi identity $\mathcal{D}_{t}\mathrm{F}_{t}=0$. The
form $\mathrm{O}$ is tensorial and since $\left\langle \mathrm{O}%
\wedge\mathrm{F}_{t}^{n}\right\rangle $ is an invariant polynomial, it is
projectable. This means that $\mathcal{D}_{t}\left\langle \mathrm{O}%
\wedge\mathrm{F}_{t}^{n}\right\rangle =d_{\mathcal{P}}\left\langle
\mathrm{O}\wedge\mathrm{F}_{t}^{n}\right\rangle $ and therefore we write%
\begin{equation}
\left\langle \mathrm{F}^{n+1}\right\rangle -\left\langle \mathrm{\bar{F}%
}^{n+1}\right\rangle =d_{\mathcal{P}}\mathrm{T}_{\mathrm{\omega}%
\leftarrow\mathrm{\bar{\omega}}}^{\left(  2n+1\right)  }%
\end{equation}
with%
\begin{equation}
\mathrm{T}_{\mathrm{\omega}\leftarrow\mathrm{\bar{\omega}}}^{\left(
2n+1\right)  }=\left(  n+1\right)  \int_{0}^{1}dt\left\langle \mathrm{O}%
\wedge\mathrm{F}_{t}^{n}\right\rangle .\label{pr23}%
\end{equation}

The $\left(  2n+1\right)  -$form $\mathrm{T}_{\mathrm{\omega}\leftarrow
\mathrm{\bar{\omega}}}^{\left(  2n+1\right)  }$ defined over the principal bundle $\mathcal{P}$ is
called \textit{Transgression form}. The transgression form is projectable over
the base space $\mathcal{M}$%
\begin{align}
T_{\mathcal{A}_{\alpha}\leftarrow\mathcal{\bar{A}}_{\alpha}}^{\left(
2n+1\right)  } &  =\sigma_{\alpha}^{\ast}\mathrm{T}_{\mathrm{\omega}%
\leftarrow\mathrm{\bar{\omega}}}^{\left(  2n+1\right)  },\nonumber \\
&  =\left(  n+1\right)  \int_{0}^{1}dt\left\langle  \Theta_{\alpha
} \wedge \left[  \mathcal{F}_{t}\right]_{\alpha}^{n}\right\rangle , \label{transform}
\end{align}
with
\begin{align*}
\Theta_{\alpha} &  =\sigma_{\alpha}^{\ast}\mathrm{O}\text{,}\\
\left[  \mathcal{F}_{t}\right]  _{\alpha} &  =\sigma_{\alpha}^{\ast}%
\mathrm{F}_{t}.
\end{align*}
The form $T_{\mathcal{A}_{\alpha}\leftarrow\mathcal{\bar{A}}_{\alpha}%
}^{\left(  2n+1\right)  }$ is called transgression over the base space or
simply transgression if there is no room for confusion. The transgression form
is globally defined so it will be denoted simply by $T_{\mathcal{A}%
\leftarrow\mathcal{\bar{A}}}^{\left(  2n+1\right)  }$. Note that over the base
space $\mathcal{M}$, the relation
\begin{equation}
\left\langle \mathcal{F}^{n+1}\right\rangle -\left\langle \mathcal{\bar{F}%
}^{n+1}\right\rangle =d_{\mathcal{M}}T_{\mathcal{A}\leftarrow\mathcal{\bar{A}%
}}^{\left(  2n+1\right)  }\label{pr26}%
\end{equation}
holds.
\end{proof}

\subsection{Chern--Simons forms} \label{chssect}

It is important to emphasize that over the principal bundle $\mathcal{P}$ the
form $\left\langle \mathrm{F}^{n+1}\right\rangle $ is not only closed but
exact. However, this is not true for $\left\langle \mathcal{F}^{n+1}%
\right\rangle $ as we will see shortly.

In the definition of the transgression form eq.$\left(  \ref{pr23}\right)  $,
two one--form connections $\mathrm{\omega}$ and $\mathrm{\bar{\omega}}$ were
used to construct a third one $\mathrm{\omega}_{t}$ given in eq.$\left(
\ref{pr24}\right)  $. It is interesting to observe that a connection over
$\mathcal{P}$ cannot be zero; otherwise it would not satisfy eq.$\left(
\ref{pr4}\right)  $. Thus, to impose the condition $\mathrm{\bar{\omega}}=0$
would mean that the expressions for $\mathrm{\omega}_{t}$ and $\mathrm{F}_{t}$
$\left[  \text{see eq}.\left(  \ref{pr24},\ref{pr25}\right)  \right]  $
\begin{align*}
\mathrm{\omega}_{t} &  =t\mathrm{\omega},\\
\mathrm{F}_{t} &  =td_{\mathcal{P}}\mathrm{\omega}+t^{2}\mathrm{\omega}%
\wedge\mathrm{\omega},
\end{align*}
no longer correspond to a one--form connection and a two--form curvature over
$\mathcal{P}$. However, the procedure used in the second half of the proof of
the Chern--Weil theorem still holds. In that case, let us to write%
\begin{equation*}
\left\langle \mathrm{F}^{n+1}\right\rangle =d_{\mathcal{P}}\mathrm{Q}^{\left(
2n+1\right)  }\left(  \mathrm{\omega}\right)  ,
\end{equation*}
where%
\begin{align*}
\mathrm{Q}^{\left(  2n+1\right)  }\left(  \mathrm{\omega}\right)   &
=\mathrm{T}_{\mathrm{\omega}\leftarrow\mathrm{0}}^{\left(  2n+1\right)  },\\
&  =\left(  n+1\right)  \int_{0}^{1}dt\left\langle \mathrm{\omega}%
\wedge\left(  td_{\mathcal{P}}\mathrm{\omega}+t^{2}\mathrm{\omega}%
\wedge\mathrm{\omega}\right)  \right\rangle ,
\end{align*}
is called the \textit{Chern--Simons} form over $\mathcal{P}$. Again, since
$\mathrm{\omega}_{t}$ and $\mathrm{F}_{t}$ are not proper connection and
curvature on $\mathcal{P}$ respectively, the Chern--Simons form it is not
invariant and therefore not projectable over the base space $\mathcal{M}$.

In other words, given two local sections $\sigma_{\alpha}:U_{\alpha}%
\subset\mathcal{M}\rightarrow\mathcal{P}$ and $\sigma_{\beta}:U_{\beta
}\subset\mathcal{M}\rightarrow\mathcal{P}$, in general must occur that%
\begin{equation*}
\sigma_{\alpha}^{\ast}\mathrm{Q}^{\left(  2n+1\right)  }\neq\sigma_{\beta
}^{\ast}\mathrm{Q}^{\left(  2n+1\right)  }.
\end{equation*}
In this way, the definition of the Chern--Simons form over the base space $\mathcal{M}$
\begin{align*}
Q_{\alpha}^{\left(  2n+1\right)  }\left(  \mathcal{A}_{\alpha}\right)   &
=\sigma_{\alpha}^{\ast}\mathrm{Q}^{\left(  2n+1\right)  }\left(
\mathrm{\omega}\right)  \\
&  =\left(  n+1\right)  \int_{0}^{1}dt\left\langle \mathcal{A}_{\alpha}%
\wedge\left(  td_{\mathcal{M}}\mathcal{A}_{\alpha}+t^{2}\mathcal{A}_{\alpha
}\wedge\mathcal{A}_{\alpha}\right)  \right\rangle
\end{align*}
it is only \textit{locally} defined over a particular open set $U_{\alpha}%
\in\mathcal{M}$. Consequently, $\left\langle \mathcal{F}^{n+1}\right\rangle $
can be written as the exterior derivative of the Chern--Simons form
$Q_{\alpha}^{\left(  2n+1\right)  }$ only in an open region $U_{\alpha}\in\mathcal{M}$
\begin{equation}
\left.  \left\langle \mathcal{F}^{n+1}\right\rangle \right\vert _{U_{\alpha}%
}=d_{\mathcal{M}}Q_{\alpha}^{\left(  2n+1\right)  } \label{csclo}
\end{equation}
but not globally over $\mathcal{M}$. In the future, we omit the index $\alpha$ in
order to avoid overloaded notation. However, it is important to keep in mind
that the Chern--Simons form it is only locally defined.

\section{Homotopy}

Another interesting property of transgression forms is that the following expression
vanishes identically
\begin{align*}
dT_{\mathcal{A}\leftarrow\mathcal{\tilde{A}}}^{\left(  2n+1\right)
}+dT_{\mathcal{\tilde{A}}\leftarrow\mathcal{\bar{A}}}^{\left(  2n+1\right)
}+dT_{\mathcal{\bar{A}}\leftarrow\mathcal{A}}^{\left(  2n+1\right)  } &
=\left\langle \mathcal{F}^{n+1}\right\rangle -\left\langle \mathcal{\tilde{F}%
}^{n+1}\right\rangle +\left\langle \mathcal{\tilde{F}}^{n+1}\right\rangle \\
&  -\left\langle \mathcal{\bar{F}}^{n+1}\right\rangle +\left\langle
\mathcal{\bar{F}}^{n+1}\right\rangle -\left\langle \mathcal{F}^{n+1}%
\right\rangle \\
&  =0.
\end{align*}
for independent gauge connections $\mathcal{A}$, $\mathcal{\bar{A}}$ and
$\mathcal{\tilde{A}}$ . Since $T_{\mathcal{\bar{A}}\leftarrow\mathcal{A}%
}^{\left(  2n+1\right)  }=-T_{\mathcal{A}\leftarrow\mathcal{\bar{A}}}^{\left(
2n+1\right)  }$, this means that%
\begin{equation*}
dT_{\mathcal{A}\leftarrow\mathcal{\bar{A}}}^{\left(  2n+1\right)
}=dT_{\mathcal{A}\leftarrow\mathcal{\tilde{A}}}^{\left(  2n+1\right)
}+dT_{\mathcal{\tilde{A}}\leftarrow\mathcal{\bar{A}}}^{\left(  2n+1\right)  }.
\end{equation*}
Therefore, it is always possible to decompose a transgression as the sum of
two others plus a closed form $\vartheta$%
\begin{equation*}
T_{\mathcal{A}\leftarrow\mathcal{\bar{A}}}^{\left(  2n+1\right)
}=T_{\mathcal{A}\leftarrow\mathcal{\tilde{A}}}^{\left(  2n+1\right)
}+T_{\mathcal{\tilde{A}}\leftarrow\mathcal{\bar{A}}}^{\left(  2n+1\right)
}+\vartheta.
\end{equation*}
The functional dependence of the closed form $\vartheta$ can be determined by
using a powerful tool, the \textit{Extended Homotopy Cartan formula.}

\subsection{The extended Cartan homotopy formula \textrm{ECHF}}

Consider now a set of $(r+2)$ independent gauge connections $\mathcal{A}%
_{i}\in\Omega^{1}\left(  \mathcal{M}\right)  \otimes\mathfrak{g}$ with
$i=0,...,r+1$. Moreover, let us consider the embedding of the $(r+1)$ simplex $T_{r+1}$ in $\mathbb{R}^{r+2}$ defined by
\begin{equation*}
\begin{tabular}{c c c c}
$\{(t^0,t^1, \ldots,t^{r+1}) \in \mathbb{R}^{r+2}$, & 
with& $t^i\geqslant 1, \forall i=1, \ldots, r+1$ and& $\sum\limits_{i=0}^{r+1}t^i=1\}$
\end{tabular}
\end{equation*}
 The relation between the simplex and the set of gauge connections is such that the expression
\begin{equation*}
\mathcal{A}_{t}=\sum\limits_{i=0}^{r+1}t^{i}\mathcal{A}_{i}%
\end{equation*}
transforms as a gauge connection when $(t^0,t^1, \ldots,t^{r+1})\in T_{r+1}$. It is direct to verify that if one performs a gauge transformation to each $\mathcal{A}_{i}$, then $\mathcal{A}_{t}$ transforms as a connection. This
allow us to define a two--form curvature $\mathcal{F}_{t}=d\mathcal{A}%
_{t}+\mathcal{A}_{t}\wedge\mathcal{A}_{t}$. 
Thus, for every point of the simplex $T_{r+1}$, we associate a connection $\mathcal{A}_i$. In particular, the $i$-th vertex of $T_{r+1}$ is related to
$i$-th connection $\mathcal{A}_{i}$. We denote the simplex of the associated gauge connections by
\begin{equation*}
T_{r+1}=\left(  \mathcal{A}_{0}\mathcal{A}_{1}...\mathcal{A}_{r+1}\right).
\end{equation*}

Let $\Upsilon$ be a polynomial in the forms $\left\{  \mathcal{A}%
_{t},\mathcal{F}_{t},d_{t}\mathcal{A}_{t},d_{t}\mathcal{F}_{t}\right\}  $
which is also a $\left(  q+m\right)  -$form over $T_{r+1}\times\mathcal{M}$. Let $d$ and $d_t$ be the exterior derivative operator acting on $\mathcal{M}$ and $T_{r+1}$ respectively.
We introduce now the \textit{homotopy derivation
} operator $l_{t}$ which maps differential forms according to%
\begin{equation*}
l_{t}:\Omega^{a}\left(  \mathcal{M}\right)  \times\Omega^{b}\left(
T_{r+1}\right)  \longrightarrow\Omega^{a-1}\left(  \mathcal{M}\right)
\times\Omega^{b+1}\left(  T_{r+1}\right)  .
\end{equation*}
This operator satisfies the Leibniz rule, and together with the operators $d$
and $d_{t}$ define the following graded algebra%
\begin{align}
d^{2} &  =0,\label{pr27}\\
d_{t}^{2} &  =0,\label{pr28}\\
\left[  l_{t},d\right]   &  =d_{t},\label{pr29}\\
\left\{  d,d_{t}\right\}   &  =0.\label{pr30}%
\end{align}
A consistent way to define the action of $l_{t}$ over $\mathcal{A}_{t}$ and $\mathcal{F}_{t}$ is the following%
\begin{align*}
l_{t}\mathcal{F}_t &  =d_{t}\mathcal{A}_{t},\\
l_{t}\mathcal{A}_{t} &  =0.
\end{align*}

Using eq.$\left(  \ref{pr27}-\ref{pr30}\right)  $ it is possible to show that%
\begin{equation*}
\left[  l_{t}^{p+1},d\right]  \Upsilon=\left(  p+1\right)  d_{t}l_{t}%
^{p}\Upsilon.
\end{equation*}
Now, integrating over the simplex $T_{r+1}$ with $p+q=r$, we have%
\begin{align}
\int_{T_{r+1}}l_{t}^{p+1}d\Upsilon-\int_{T_{r+1}}dl_{t}^{p+1}\Upsilon &
=\left(  p+1\right)  \int_{T_{r+1}}d_{t}l_{t}^{p}\Upsilon,\nonumber\\
& =\left(  p+1\right)  \int_{\partial T_{r+1}}l_{t}^{p}\Upsilon.\label{pr31}%
\end{align}
Since $l_{t}^{p+1}\Upsilon$ is a $\left(  r+1\right)  -$form over $T_{r+1}$,
it follows%
\begin{equation*}
\int_{T_{r+1}}dl_{t}^{p+1}\Upsilon=\left(  -1\right)  ^{r+1}d\int_{T_{r+1}%
}l_{t}^{p+1}\Upsilon
\end{equation*}
Replacing in eq.$\left(  \ref{pr31}\right)  $ and introducing normalization
factors we have%
\begin{equation}
\int_{\partial T_{r+1}}\frac{1}{p!}l_{t}^{p}\Upsilon=\int_{T_{r+1}}\frac
{1}{\left(  p+1\right)  !}l_{t}^{p+1}d\Upsilon+\left(  -1\right)  ^{r}%
d\int_{T_{r+1}}\frac{1}{\left(  p+1\right)  !}l_{t}^{p+1}\Upsilon.\label{pr32}%
\end{equation}
This important result it is known in literature as the \textit{Extended
Homotopy Cartan Formula }(\textrm{EHCF}) \cite{Manes:2012zz}\cite{Izaurieta:2006wv}\cite{Izaurieta:2005vp}.

Let us look now at the particular case where the following polynomial is
selected%
\begin{equation*}
\Upsilon=\left\langle \mathcal{F}_{t}^{n+1}\right\rangle .
\end{equation*}
This choice carries three properties
\begin{enumerate}
\item $\Upsilon$ is $\mathcal{M}-$closed,
\item $\Upsilon$ is a $0-$form on $T_{r+1}$ i.e, $q=0$,
\item $\Upsilon$ is a $\left(  2n+2\right)  -$form on $\mathcal{M}$. Thus, $0\leqslant p \leqslant 2n+2$.
\end{enumerate}

With these considerations
\textrm{EHCF} reduces to%
\begin{equation}
\int_{\partial T_{p+1}}\frac{l_{t}^{p}}{p!}\left\langle \mathcal{F}_{t}%
^{n+1}\right\rangle =\left(  -1\right)  ^{p}d\int_{T_{p+1}}\frac{l_{t}^{p+1}%
}{\left(  p+1\right)  !}\left\langle \mathcal{F}_{t}^{n+1}\right\rangle,
\end{equation}
which is known as the restricted or closed version of \textrm{EHCF}.

\subsubsection{$p=0$, the Chern-Weil theorem}

A well known particular case of \textrm{EHCF} is the Chern--Weil theorem.
Setting $p=0$ in the above expression, we get%
\begin{equation}
\int_{\partial T_{1}}\left\langle \mathcal{F}_{t}^{n+1}\right\rangle
=d\int_{T_{1}}l_{t}\left\langle \mathcal{F}_{t}^{n+1}\right\rangle
\label{ch2.jojo}%
\end{equation}
where $\mathcal{F}_{t}$ is the curvature for the connection $\mathcal{A}%
_{t}=t_{0}\mathcal{A}_{0}+t_{1}\mathcal{A}_{1}$ where $t_{0}+t_{1}=1$. The
boundary of the simplex $T_{1}=\left(  \mathcal{A}_{0},\mathcal{A}_{1}\right)
$ corresponds to%
\begin{equation*}
\partial\left(  \mathcal{A}_{0},\mathcal{A}_{1}\right)  =\left(
\mathcal{A}_{1}\right)  -\left(  \mathcal{A}_{0}\right)  ,
\end{equation*}
so the left hand side of eq.$\left(  \ref{ch2.jojo}\right)  $ is then%
\begin{equation*}
\int_{\partial T_{1}}\left\langle \mathcal{F}_{t}^{n+1}\right\rangle
=\left\langle \mathcal{F}_{1}^{n+1}\right\rangle -\left\langle \mathcal{F}%
_{0}^{n+1}\right\rangle .
\end{equation*}
Since $\left\langle \mathcal{F}_{t}^{n+1}\right\rangle $ is a symmetric
polynomial, we have
\begin{equation*}
l_{t}\left\langle \mathcal{F}_{t}^{n+1}\right\rangle =\left(  n+1\right)
\left\langle l_{t}\mathcal{F}_{t}\mathcal{F}_{t}^{n}\right\rangle .
\end{equation*}
Now, the homotopic derivative of the curvature $l_{t}\mathcal{F}_{t}$ is given
by
\begin{align*}
l_{t}\mathcal{F}_{t} &  =d_{t}\mathcal{A}_{t},\\
&  =dt^{0}\mathcal{A}_{0}+dt^{1}\mathcal{A}_{1},\\
&  =dt^{1}\left(  \mathcal{A}_{1}-\mathcal{A}_{0}\right)  .
\end{align*}
In this way,%
\begin{equation}
l_{t}\left\langle \mathcal{F}_{t}^{n+1}\right\rangle =\left(  n+1\right)
dt^{1}\left\langle \left(  \mathcal{A}_{1}-\mathcal{A}_{0}\right)
\wedge\mathcal{F}_{t}^{n}\right\rangle .\label{pr33}%
\end{equation}
Replacing in eq.$\left(  \ref{ch2.jojo}\right)  $ we obtain the Chern--Weil
theorem%
\begin{align*}
\left\langle \mathcal{F}_{1}^{n+1}\right\rangle -\left\langle \mathcal{F}%
_{0}^{n+1}\right\rangle  &  =\left(  n+1\right)  d\int_{0}^{1}dt\left\langle
\left(  \mathcal{A}_{1}-\mathcal{A}_{0}\right)  \wedge\mathcal{F}_{t}%
^{n}\right\rangle ,\\
&  =dT_{\mathcal{A}_{1}\leftarrow\mathcal{A}_{0}}^{\left(  2n+1\right)  }.
\end{align*}


\subsubsection{$p=1$, the Triangle Equation} \label{tria}

The $p=1$ case corresponds to the so called triangle equation. In fact, for
$p=1$ \textrm{EHCF} reads%
\begin{equation}
\int_{\partial T_{2}}l_{t}\left\langle \mathcal{F}_{t}^{n+1}\right\rangle
=-\frac{1}{2}d\int_{T_{2}}l_{t}^{2}\left\langle \mathcal{F}_{t}^{n+1}%
\right\rangle, \label{ch2.2klkl}%
\end{equation}
where $\mathcal{F}_{t}$ is the curvature for the connection $\mathcal{A}%
_{t}=t_{0}\mathcal{A}_{0}+t_{1}\mathcal{A}_{1}+t_{2}\mathcal{A}_{2},$ with
$t_{0}+t_{1}+t_{2}=1$. Again, the boundary of the simplex $T_{2}=\left(
\mathcal{A}_{0},\mathcal{A}_{1},\mathcal{A}_{2}\right)  $ corresponds to%
\begin{equation*}
\partial\left(  \mathcal{A}_{0},\mathcal{A}_{1},\mathcal{A}_{2}\right)
=\left(  \mathcal{A}_{1}\mathcal{A}_{2}\right)  -\left(  \mathcal{A}%
_{0}\mathcal{A}_{2}\right)  +\left(  \mathcal{A}_{0}\mathcal{A}_{1}\right)  ,
\end{equation*}
and the left hand side in eq.$\left(  \ref{ch2.2klkl}\right)  $ is given by%
\begin{equation*}
\int_{\partial T_{2}}l_{t}\left\langle \mathcal{F}_{t}^{n+1}\right\rangle
=\int_{\left(  \mathcal{A}_{1}\mathcal{A}_{2}\right)  }l_{t}\left\langle
\mathcal{F}_{t}^{n+1}\right\rangle -\int_{\left(  \mathcal{A}_{0}%
\mathcal{A}_{2}\right)  }l_{t}\left\langle \mathcal{F}_{t}^{n+1}\right\rangle
+\int_{\left(  \mathcal{A}_{0}\mathcal{A}_{1}\right)  }l_{t}\left\langle
\mathcal{F}_{t}^{n+1}\right\rangle .
\end{equation*}
Since $\left[  \text{see eq.}\left(  \ref{pr33}\right)  \right]  $%
\begin{equation*}
\int_{\left(  \mathcal{A}_{1}\mathcal{A}_{2}\right)  }l_{t}\left\langle
\mathcal{F}_{t}^{n+1}\right\rangle =Q_{\mathcal{A}_{2}\leftarrow
\mathcal{A}_{1}}^{\left(  2n+1\right)  },
\end{equation*}
it follows%
\begin{equation}
\int_{\partial T_{2}}l_{t}\left\langle \mathcal{F}_{t}^{n+1}\right\rangle
=T_{\mathcal{A}_{2}\leftarrow\mathcal{A}_{1}}^{\left(  2n+1\right)
}-T_{\mathcal{A}_{2}\leftarrow\mathcal{A}_{0}}^{\left(  2n+1\right)
}+T_{\mathcal{A}_{1}\leftarrow\mathcal{A}_{0}}^{\left(  2n+1\right)
}.\label{ch2.2.ttt}%
\end{equation}
Now, using the symmetry of the polynomial $\left\langle ...\right\rangle $ one
derives%
\begin{equation}
\frac{1}{2}l_{t}^{2}\left\langle \mathcal{F}_{t}^{n+1}\right\rangle =\frac
{1}{2}n\left(  n+1\right)  \left\langle \left(  d_{t}\mathcal{A}_{t}\right)
^{2}\wedge\mathcal{F}_{t}^{n+1}\right\rangle ,\label{ch2.2.popo}%
\end{equation}
where%
\begin{equation*}
d_{t}\mathcal{A}_{t}=dt^{0}\mathcal{A}_{0}+dt^{1}\mathcal{A}_{1}%
+dt^{2}\mathcal{A}_{2,}%
\end{equation*}
but considering that
\begin{equation*}
dt^{0}+dt^{1}+dt^{2}=0
\end{equation*}
one finds%
\begin{equation*}
d_{t}\mathcal{A}_{t}=dt^{0}\left(  \mathcal{A}_{0}-\mathcal{A}_{1}\right)
+dt^{2}\left(  \mathcal{A}_{2}-\mathcal{A}_{1}\right)
\end{equation*}
Replacing in eq.$\left(  \ref{ch2.2.popo}\right)  $ we obtain%
\begin{equation*}
\frac{1}{2}l_{t}^{2}\left\langle \mathcal{F}_{t}^{n+1}\right\rangle =-n\left(
n+1\right)  dt^{0}dt^{2}\left\langle \left(  \mathcal{A}_{2}-\mathcal{A}%
_{1}\right)  \wedge\left(  \mathcal{A}_{1}-\mathcal{A}_{0}\right)
\wedge\mathcal{F}_{t}^{n+1}\right\rangle
\end{equation*}
It is convenient to re-define the integration parameters%
\begin{align*}
t &  =1-t^{1},\\
s &  =t^{2},
\end{align*}
and integrate explicitly over $T_{2}$. In this way, we get
\begin{equation*}
\frac{1}{2}\int_{\partial T_{2}}l_{t}^{2}\left\langle \mathcal{F}_{t}%
^{n+1}\right\rangle =Q_{\mathcal{A}_{2}\leftarrow\mathcal{A}_{1}%
\leftarrow\mathcal{A}_{0}}^{\left(  2n\right)  }%
\end{equation*}
where $Q_{\mathcal{A}_{2}\leftarrow\mathcal{A}_{1}\leftarrow\mathcal{A}_{0}%
}^{\left(  2n\right)  }$ is defined as%
\begin{equation*}
Q_{\mathcal{A}_{2}\leftarrow\mathcal{A}_{1}\leftarrow\mathcal{A}_{0}}^{\left(
2n\right)  }=n\left(  n+1\right)  \int_{0}^{1}dt\int_{0}^{t}ds\left\langle
\left(  \mathcal{A}_{2}-\mathcal{A}_{1}\right)  \wedge\left(  \mathcal{A}%
_{1}-\mathcal{A}_{0}\right)  \wedge\mathcal{F}_{st}^{n-1}\right\rangle .
\end{equation*}
Inserting this expression in eq.$\left(  \ref{ch2.2.ttt}\right)  $ the
triangle equations is finally obtained%
\begin{equation}
\ T_{\mathcal{A}_{2}\leftarrow\mathcal{A}_{0}}^{\left(  2n+1\right)
}=T_{\mathcal{A}_{2}\leftarrow\mathcal{A}_{1}}^{\left(  2n+1\right)
}+T_{\mathcal{A}_{1}\leftarrow\mathcal{A}_{0}}^{\left(  2n+1\right)
}+dQ_{\mathcal{A}_{2}\leftarrow\mathcal{A}_{1}\leftarrow\mathcal{A}_{0}%
}^{\left(  2n\right)  }.\label{pr34}%
\end{equation}
As we will see in the following chapter, eq.$\left(  \ref{pr34}\right)  $ is
extremely useful from the point of view that transgression forms will be used
as Lagrangians functions for constructing physical theories. For this reason, it is of
vital importance to split the transgression in different parts each of them corresponding
to different interactions present in the theory.

==> Design.tex <==

\chapter{Transgression forms as source of gauge theories}
\label{ch:Transgression}

Given a certain symmetry, the natural way to construct a gauge invariant
theory is by using a Yang-Mills Lagrangian. This is for instance the case of
the interactions of the Standard Model, the most successful and remarkable
model in particle physics. The Yang--Mills action is given by%
\begin{equation}
\mathsf{S}_{\mathrm{YM}}=-\frac{1}{4}\int_{\mathcal{M}}\sqrt{g}%
\text{\textbf{Tr}}\left(  \mathcal{F}^{\mu\nu}\mathcal{F}_{\mu\nu}\right)
d^{4}x. \label{tr1}%
\end{equation}
However, it is not so hard to face some limitations. As it can be seen from
eq.$\left(  \ref{tr1}\right)  $, the Yang-Mills action requires the inclusion
of a metric structure as a background. Thus, in the case of a curved base
space $\mathcal{M}$, the metric tensor becomes dynamical and the action cannot
be considered as describing a pure gauge theory due to the inclusion of a
dynamic field which it is not part of the gauge connection $\mathcal{A}$.

For this reason it seems natural to think in gauge theories which are
background independent. Transgression forms are natural candidates for
``metric-free" actions in the sense that they can be used to construct gauge
theories without any associated background. The scenario is still better:
Transgressions forms are genuinely gauge invariant objects, they are also
globally defined, so they can be integrated over the whole base space
$\mathcal{M}$. The price to pay is the inclusion, in addition to the gauge
field $\mathcal{A}$, a second one--form connection $\mathcal{\bar{A}}$. This
duplicity in the gauge fields could be thought as an obstruction from a
traditional point of view. However, we will see that the presence of two gauge
connections is a very versatile feature. In fact, we will see how
transgression actions give rise to different types of theories depending on
the conditions imposed on the connections $\mathcal{A}$ and $\mathcal{\bar{A}%
}$.

Throughout this chapter, the consequences of these possible elections are
explored. First, we consider the most general transgression field theory. That is, without imposing any condition on the
connections. Secondly, we show that transgressions forms conduce to Chern--Simons theory by imposing 
$\mathcal{\bar{A}}=0$, and we will present as an example the constructions of Chern--Simons gravitational theories in odd dimensions. Finally, we study the case when both gauge
connections are related by a gauge transformation. In this case we will show
that the resulting theory is the so called
gauged Wess--Zumino--Witten action. For more details about some of the results
presented in this section, see \cite{Borowiec:2003rd}\cite{Borowiec:2005ky}\cite{Mora:2003wy}\cite{Miskovic:2004us}.

\section{Transgressions forms as Lagrangians}

\begin{definition}
Let $\mathcal{P}$ be a principal bundle with a $\left(  2n+1\right)
-$dimensional orientable base space $\mathcal{M}$. Let $\mathcal{A}$ and
$\mathcal{\bar{A}}$ be two Lie valued connections over $\mathcal{M}$, and let
$T_{\mathcal{A}\leftarrow\mathcal{\bar{A}}}^{\left(  2n+1\right)  }$ be the
transgression form over the base space $\mathcal{M}$ eq.$(\ref{transform})$
\begin{equation*}
T_{\mathcal{A}\leftarrow\mathcal{\bar{A}}}^{\left(  2n+1\right)  }=\left(
n+1\right)  \int_{0}^{1}dt\left\langle \Theta\wedge\mathcal{F}_{t}%
^{n}\right\rangle .
\end{equation*}
We define as the Transgression Lagrangian over $\mathcal{M}$, to the $\left(
2n+1\right)  -$form
\begin{align}
\mathsf{L}_{\mathsf{T}}^{\left(  2n+1\right)  }\left(  \mathcal{A}%
,\mathcal{\bar{A}}\right)   &  =\kappa T_{\mathcal{A}\leftarrow\mathcal{\bar
{A}}}^{\left(  2n+1\right)  }\nonumber\\
&  =\kappa\left(  n+1\right)  \int_{0}^{1}dt\left\langle \Theta\wedge
\mathcal{F}_{t}^{n}\right\rangle \label{ch2transl}%
\end{align}
where $\kappa$ is a constant, $\Theta=\mathcal{A}$ $-\mathcal{\bar{A}}$, and
$\mathcal{F}_{t}=d\mathcal{A}_{t}+\mathcal{A}_{t}\wedge\mathcal{A}_{t}$ is the
curvature of $\mathcal{A}_{t}=\mathcal{\bar{A}}+t\Theta$.
\end{definition}

It is direct to show that the transgression Lagrangian eq.$\left(
\ref{ch2transl}\right)  $ is gauge invariant. In fact under gauge
transformations%
\begin{align}
\mathcal{A}  &  \rightarrow\mathcal{A}^{\prime}=g^{-1}\mathcal{A}%
g+g^{-1}dg\label{ch2gin1}\\
\mathcal{\bar{A}}  &  \rightarrow\mathcal{\bar{A}}^{\prime}=g^{-1}%
\mathcal{\bar{A}}g+g^{-1}dg \label{ch2gin2}%
\end{align}
with $g\left(  x\right)  =\exp\left\{  \lambda^{A}\left(  x\right)
\mathrm{T}_{A}\right\}  \in\mathcal{G}$ and $\left\{  \mathrm{T}%
_{A},A=1,...,\dim\left(  \mathfrak{g}\right)  \right\}  ,$we have
\begin{align*}
\Theta &  \longrightarrow\Theta^{\prime}=g^{-1}\Theta g,\\
\mathcal{F}_{t}  &  \longrightarrow\mathcal{F}_{t}^{\prime}=g^{-1}%
\mathcal{F}_{t}g.
\end{align*}
Using the invariance property of $\left\langle \ldots\right\rangle $
eq.$(\ref{pr21})$, it follows%
\begin{equation*}
\mathsf{L}_{\mathsf{T}}^{\left(  2n+1\right)  }\left(  \mathcal{A}%
,\mathcal{\bar{A}}\right)  =\mathsf{L}_{\mathsf{T}}^{\left(  2n+1\right)
}\left(  \mathcal{A}^{\prime},\mathcal{\bar{A}}^{\prime}\right)  .
\end{equation*}

The transgression Lagrangian satisfy two properties
\begin{itemize}
\item Antisymmetry%
\begin{equation*}
\mathsf{L}_{\mathsf{T}}^{\left(  2n+1\right)  }\left(  \mathcal{A}%
,\mathcal{\bar{A}}\right)  =-\mathsf{L}_{\mathsf{T}}^{\left(  2n+1\right)
}\left(  \mathcal{\bar{A}},\mathcal{A}\right)  .
\end{equation*}

\item Triangle Equation [see Section $(\ref{tria})$]%
\begin{equation}
\mathsf{L}_{\mathsf{T}}^{\left(  2n+1\right)  }\left(  \mathcal{A}%
,\mathcal{\bar{A}}\right)  =T_{\mathcal{A\leftarrow\tilde{A}}}^{\left(
2n+1\right)  }-T_{\mathcal{\bar{A}\leftarrow\tilde{A}}}^{\left(  2n+1\right)
}-dQ_{\mathcal{A\leftarrow\bar{A}\leftarrow\tilde{A}}}^{\left(  2n\right)  }.
\label{ch2trian}%
\end{equation}

\end{itemize}

It is interesting to note that imposing $\mathcal{\tilde{A}}=0$ in eq.$\left(
\ref{ch2trian}\right)  $ does not affect the globality of $\mathsf{L}%
_{\mathsf{T}}^{\left(  2n+1\right)  }\left(  \mathcal{A},\mathcal{\bar{A}%
}\right)  $. This is mainly because the definition of $\mathsf{L}_{\mathsf{T}%
}^{\left(  2n+1\right)  }\left(  \mathcal{A},\mathcal{\bar{A}}\right)  $ does
not depend on the election of $\mathcal{\tilde{A}}$.

On the other hand, since $Q^{\left(  2n+1\right)  }\left(  \mathcal{A}\right)
=T_{\mathcal{A}\leftarrow0}^{\left(  2n+1\right)  }$ corresponds to the
Chern--Simons form locally defined over $\mathcal{M}$, it is natural to define
the Chern--Simons Lagrangian as%
\begin{align}
\mathsf{L}_{\mathsf{CS}}^{\left(  2n+1\right)  }\left(  \mathcal{A}\right)
&  =\kappa T_{\mathcal{A}\leftarrow0}^{\left(  2n+1\right)  },\nonumber\\
&  =\kappa\left(  n+1\right)  \int_{0}^{1}dt\left\langle \mathcal{A\wedge
}\left(  td\mathcal{A}+t^{2}\mathcal{A}\wedge\mathcal{A}\right)  \right\rangle
. \label{ch2csl}%
\end{align}
Thus, it is possible to write the transgression Lagrangian as the difference
of two Chern--Simons forms plus a boundary term%
\begin{equation}
\mathsf{L}_{\mathsf{T}}^{\left(  2n+1\right)  }\left(  \mathcal{A}%
,\mathcal{\bar{A}}\right)  =\mathsf{L}_{\mathsf{CS}}^{\left(  2n+1\right)
}\left(  \mathcal{A}\right)  -\mathsf{L}_{\mathsf{CS}}^{\left(  2n+1\right)
}\left(  \mathcal{\bar{A}}\right)  -\kappa dQ_{\mathcal{A\leftarrow\bar
{A}\leftarrow}0}^{\left(  2n\right)  }. \label{ch2tranlag}%
\end{equation}


It is important to remark that even when the Chern--Simons Lagrangian is only
locally defined, the transgression Lagrangian still is globally defined. This
is due to the presence of the boundary term $\kappa dQ_{\mathcal{A\leftarrow
\bar{A}\leftarrow}0}^{\left(  2n\right)  }$, which plays the role of a
regularizing term, guaranteeing the full invariance of the Lagrangian under
gauge transformations.

\section{Transgression Field Theory}

The most general transgression field theory can be constructed considering
$\mathcal{A}$ and $\mathcal{\bar{A}}$ as independent dynamic fields. In this
case, using eq.$\left(  \ref{ch2tranlag}\right)  $ we define the action%
\begin{align}
\mathsf{S}_{\mathsf{T}}^{\left(  2n+1\right)  }\left[  \mathcal{A}%
,\mathcal{\bar{A}}\right]   &  =\int_{\mathcal{M}}\mathsf{L}_{\mathsf{T}%
}^{\left(  2n+1\right)  }\left(  \mathcal{A},\mathcal{\bar{A}}\right)
\nonumber\\
&  =\int_{\mathcal{M}}\mathsf{L}_{\mathsf{CS}}^{\left(  2n+1\right)  }\left(
\mathcal{A}\right)  -\int_{\mathcal{M}}\mathsf{L}_{\mathsf{CS}}^{\left(
2n+1\right)  }\left(  \mathcal{\bar{A}}\right)  -\kappa d\int_{\mathcal{M}%
}Q_{\mathcal{A\leftarrow\bar{A}\leftarrow}0}^{\left(  2n\right)
}.\label{ch2tranact}%
\end{align}
In this context we have constructed a gauge theory composed by two
auto-interacting gauge fields $\mathcal{A}$ and $\mathcal{\bar{A}}$ at the
bulk $\mathcal{M}$, but interacting between them at the boundary
$\partial\mathcal{M}$.

There are two independent set of symmetries lurking in the transgression
action eq.$\left(  \ref{ch2tranact}\right)  $. The first one is a built-in
symmetry, guaranteed from the outset by our use of differential forms
throughout: it is diffeomorphism invariance%
\begin{align}
\delta_{\text{{\scriptsize diff}}}\mathcal{A}  &  =-\pounds _{\xi}%
\mathcal{A},\label{ch2diffa}\\
\delta_{\text{{\scriptsize diff}}}\mathcal{\bar{A}}  &  =-\pounds _{\xi
}\mathcal{\bar{A}},\nonumber
\end{align}
where $\pounds $ is the Lie derivative operator, and $\xi$ is a vector field
that generates the infinitesimal diffeomorphism.

The second symmetry is gauge symmetry. Under a continuous local gauge
transformation with element $g=\exp\left\{  \lambda^{A}\mathrm{T}_{A}\right\}
$, the gauge connections $\mathcal{A}$ and $\mathcal{\bar{A}}$ change
according to eq.$\left(  \ref{ch2gin1},\ref{ch2gin2}\right)  $. In an
infinitesimal form, these gauge transformations are given by%
\begin{align}
\delta_{\text{{\scriptsize gauge}}}\mathcal{A}  &  =D_{\mathcal{A}}%
\lambda,\label{ch2gaugetr}\\
\delta_{\text{{\scriptsize gauge}}}\mathcal{\bar{A}}  &  =D_{\mathcal{\bar{A}%
}}\lambda,\nonumber
\end{align}
where $\lambda=\lambda^{A}\mathrm{T}_{A}$ is a $\mathfrak{g}-$valued $0-$form
group parameter.

The variation of the transgression action eq.$\left(  \ref{ch2tranact}\right)
$ leads to the following equation of motion%
\begin{align*}
\left\langle \mathrm{T}_{A}\mathcal{F}^{n}\right\rangle  &  =0,\\
\left\langle \mathrm{T}_{A}\mathcal{\bar{F}}^{n}\right\rangle  &  =0,
\end{align*}
subject to the boundary conditions%
\begin{equation*}
\left.  \int_{0}^{1}dt\left\langle \delta\mathcal{A}_{t}\wedge\Theta
\wedge\mathcal{F}_{t}^{n-1}\right\rangle \right\vert _{\partial\mathcal{M}%
}=0.
\end{equation*}


\section{Chern--Simons theory}

Using Chern--Simons forms as Lagrangians seems to be the most direct way to
avoid using two gauge connections. In fact, the Chern--Simons Lagrangian
eq.$\left(  \ref{ch2csl}\right)  $ depends only of a single dynamical field
$\mathcal{A}$. However, the simplification of imposing $\mathcal{\bar{A}}=0$
in the transgression Lagrangian eq.$\left(  \ref{ch2transl}\right)  $ give
raise to nontrivial problems. As it was mentioned in section \ref{chssect},
Chern--Simons forms are only locally defined over the base space $\mathcal{M}%
$. This means that, if $\left\{  U_{\alpha}\right\}  $ is an open overing of a
$\left(  2n+1\right)  -$dimensional base space $\mathcal{M}$, on the nonempty
intersection $U_{\alpha}\cap U_{\beta}$ we have%
\begin{equation*}
Q_{\alpha}^{\left(  2n+1\right)  }\left(  \mathcal{A}_{\alpha}\right)  \neq
Q_{\beta}^{\left(  2n+1\right)  }\left(  \mathcal{A}_{\beta}\right)  .
\end{equation*}
This nonlocality property of the Chern--Simons form is a source of ambiguity
in the definition of the action. The reason is basically that integrating
$\left.  \mathsf{L}_{\mathsf{CS}}^{\left(  2n+1\right)  }\right\vert
_{U_{\alpha}}=\kappa Q_{\alpha}^{\left(  2n+1\right)  }$ and $\left.
\mathsf{L}_{\mathsf{CS}}^{\left(  2n+1\right)  }\right\vert _{U_{\beta}%
}=\kappa Q_{\beta}^{\left(  2n+1\right)  }$ on the intersection $U_{\alpha
}\cap U_{\beta}$, conduces in general to different answers. Therefore, it is
impossible to define the action in a unique manner.

However, in the case of Chern--Simons forms it is possible to partially
circumvent this problem. An easy way to see this is considering eq.$(\ref{csclo}) $. Since $\left\langle \mathcal{F}^{n+1}\right\rangle $ is
gauge invariant, it follows that under a gauge transformation%
\begin{equation*}
\delta_{\text{{\scriptsize gauge}}}\left\langle \mathcal{F}^{n+1}\right\rangle
=d\left(  \delta_{\text{{\scriptsize gauge}}}Q^{\left(  2n+1\right)  }\right)
=0.
\end{equation*}
Thus, the Chern--Simons form is gauge invariant modulo a total derivative.
This implies that a Chern--Simons action can be well defined only modulo
boundary terms%
\begin{equation}
\mathsf{S}_{\mathsf{CS}}^{\left(  2n+1\right)  }\left[  \mathcal{A}\right]
=\int_{\mathcal{M}}\mathsf{L}_{\mathsf{CS}}^{\left(  2n+1\right)  }\left(
\mathcal{A}\right)  +\int_{\partial\mathcal{M}}X^{\left(  2n\right)  }.
\label{ch2csact}%
\end{equation}

The variation of the Chern--Simons action eq.$\left(  \ref{ch2csact}\right)  $
gives the equations of motion associated to the connection $\mathcal{A}$%
\begin{equation*}
\left.  \left\langle \mathrm{T}_{A}\mathcal{F}^{n}\right\rangle \right\vert
_{\mathcal{M}}=0,
\end{equation*}
but in principle it is not possible to define boundary conditions starting
form the action principle. This has serious implications. For instance, the
Noether currents and conserved charges cannot be uniquely defined. For this
reason, it is more interesting to work with transgression forms. In contrast
to Chern--Simons forms, any action principle constructed using transgression as Lagrangians is uniquely defined
and conduce to finite conserved charges via Noether theorem. See \cite{Izaurieta:2006ia}\cite{Rodriguez:2006xx} for a more detailed discussion.

The Chern--Simons action eq.$(\ref{ch2csact})$is still diffeomorphism invariant, and as it was mentioned, it remains unchanged under
gauge transformations eq.$\left(  \ref{ch2gaugetr}\right)  $ modulo boundary terms.

It is important to mention that the physical properties of a Chern--Simons
theory are strongly related with the chosen Lie algebra $\mathfrak{g}$. In
principle, the Lie algebra could be composed of different subspaces which will
conduce to different sectors in the theory; each of them with a different
physical interpretation. For instance, a particular sector in the Lie algebra
could correspond to gravitational theories and some other to the presence of
fermionic fields present in the theory. Furthermore, depending on the form of
the invariant tensor, the Chern--Simons Lagrangian splits in pieces defined on the bulk of $\mathcal{M}$,
and some other pieces defined at the boundary $\partial\mathcal{M}$.

It is desirable to use a mechanism which allows to separate systematically the
Lagrangian in terms of the respective subspaces associated to the Lie algebra
and also to separate the bulk and boundary contributions. The advantage in
doing so, is that the resulting action principle can always be written in
terms of pieces which reflect the physical features of the theory. This can be
done applying the \textrm{ECHF} recursively as we will see next.

\subsection{Subspace Separation Method}

The key observation behind the subspace separation method comes from the
triangle equation
\begin{equation}
\ T_{\mathcal{A}_{2}\leftarrow\mathcal{A}_{1}}^{\left(  2n+1\right)
}=T_{\mathcal{A}_{2}\leftarrow\mathcal{A}_{0}}^{\left(  2n+1\right)
}-T_{\mathcal{A}_{1}\leftarrow\mathcal{A}_{0}}^{\left(  2n+1\right)
}-dQ_{\mathcal{A}_{2}\leftarrow\mathcal{A}_{1}\leftarrow\mathcal{A}_{0}%
}^{\left(  2n\right)  }. \label{ch2treq}%
\end{equation}

The transgression form $T_{\mathcal{A}_{2}\leftarrow\mathcal{A}_{1}}^{\left(
2n+1\right)  }$ which interpolates between the connections $\mathcal{A}_{2}$
and $\mathcal{A}_{1}$, can be decomposed as the sum of two transgressions;
$T_{\mathcal{A}_{2}\leftarrow\mathcal{A}_{0}}^{\left(  2n+1\right)  }$ which
interpolates between $\mathcal{A}_{2}$, $\mathcal{A}_{0}$, and $T_{\mathcal{A}%
_{1}\leftarrow\mathcal{A}_{0}}^{\left(  2n+1\right)  }$ interpolating between
$\mathcal{A}_{1}$, $\mathcal{A}_{0}$, plus an exact form which depends on
$\mathcal{A}_{2}$, $\mathcal{A}_{1}$ and $\mathcal{A}_{0}$. In this way, the
triangle equation allows to divide a transgression (or Chern--Simons
alternatively) Lagrangian by using an intermediary connection $\mathcal{A}_{1}$.
In this way, the iterative use of the triangle equation enable us to perform the
separation in terms of subspaces early mentioned.

Let $\mathfrak{g}$ be a Lie algebra, $\mathcal{A}$ and $\mathcal{\bar{A}}$ two
Lie valued connections and $\mathsf{L}_{\mathsf{T}}^{\left(  2n+1\right)
}\left(  \mathcal{A},\mathcal{\bar{A}}\right)  =\kappa T_{\mathcal{A}%
\leftarrow\mathcal{\bar{A}}}^{\left(  2n+1\right)  }$. The subspace separation
of the corresponding transgression Lagrangian (or Chern--Simons in the case
$\mathcal{\bar{A}}=0$), is given as follows

\begin{enumerate}
\item Split the Lie algebra $\mathfrak{g}$ in terms of subspaces  $\mathfrak{g}=V_{0}\oplus\ldots\oplus V_{p}$.

\item Write the connections in pieces valued in each subspace $\mathcal{A}%
=\mathrm{a}_{0}+\ldots+\mathrm{a}_{p}$ and $\mathcal{\bar{A}}=\mathrm{\bar{a}%
}_{0}+\ldots+\mathrm{\bar{a}}_{p}$.

\item Use the triangle equation $\left(  \ref{ch2treq}\right)  $ for writing
$\mathsf{L}_{\mathsf{T}}^{\left(  2n+1\right)  }\left(  \mathcal{A}%
,\mathcal{\bar{A}}\right)  $ (or $\mathsf{L}_{\mathsf{CS}}^{\left(
2n+1\right)  }\left(  \mathcal{A}\right)  $) with%
\begin{align*}
\mathcal{A}_{0}  &  =\mathcal{\bar{A}}\text{,}\\
\mathcal{A}_{1}  &  =\mathrm{a}_{0}+\ldots+\mathrm{a}_{p-1}\text{,}\\
\mathcal{A}_{2}  &  =\mathcal{A}\text{.}%
\end{align*}


\item Iterate step $3$ for the transgression $T_{\mathcal{A}_{1}%
\leftarrow\mathcal{A}_{0}}^{\left(  2n+1\right)  }$ and so forth.
\end{enumerate}

As an example, we show next how to write in an explicit way the Chern--Simons
Lagrangian for gravity in odd dimensions.

\subsection{An example: Chern--Simons Gravity}

In this section, we describe general aspects of how to obtain Chern--Simons
gravity in arbitrary odd dimensions, using the tools developed in the previous
sections. The motivation for considering Chern--Simons gravity through this
thesis will be given in the next chapter when the topological theories of
gravity in arbitrary dimensions will be studied. For a detailed discussion
about Chern--Simons gravity see ref\{\}\{\}\{\} (aqui usamos informacion del paper)

\section{Gauged Wess--Zumino--Witten Theory}

We have learned that the most general tansgression field theory eq.$\left(
\ref{ch2tranact}\right)  $ is globally defined. The price to pay was the
inclusion of two connections $\mathcal{A}$ and $\mathcal{\bar{A}}$ as
independent dynamic fields. This certainly opens the question about the
physical meaning of the field $\mathcal{\bar{A}}$. We also have shown that
further simplifications, like imposing $\mathcal{\bar{A}}=0$ in the
transgression action, conduces to Chern--Simons theories eq.$\left(
\ref{ch2csact}\right)  $ which are not globally defined and only gauge
invariant modulo boundary terms.

There is a third and no less interesting possibility: that is to regard
$\mathcal{A}$ and $\mathcal{\bar{A}}$ as two connections defining the same
nontrivial principal bundle $\mathcal{P}$. This means that they are related by
a gauge transformation.

If a nontrivial bundle is considered, the transgression action eq.$\left(
\ref{ch2tranact}\right)  $ it is not globally defined. However, the action can
be treated formally provided more than one chat is used. In this case, it is
necessary to introduce gauge connections defined in each chart, such that, in
the overlap of two charts $U_{\alpha}\cap U_{\beta}$ the connections are
related by
\[
\mathcal{\bar{A}}=g^{-1}\mathcal{A}g+g^{-1}dg\equiv\mathcal{A}^{g}%
\]
where $g=\tau_{\alpha\beta}\left(  x\right)  $ is a transition function which
determines the nontriviality of the principal bundle $\mathcal{P}$.

To see how the transgression action eq.$\left(  \ref{ch2tranact}\right)  $
changes under $\mathcal{\bar{A}}\longrightarrow\mathcal{A}^{g}$ we first
consider
\begin{align*}
\mathsf{L}_{\mathsf{CS}}^{\left(  2n+1\right)  }\left(  \mathcal{\bar{A}%
}\right)   &  =\mathsf{L}_{\mathsf{CS}}^{\left(  2n+1\right)  }\left(
\mathcal{A}^{g}\right)  ,\\
&  =\kappa T_{\mathcal{A}^{g}\leftarrow0}^{\left(  2n+1\right)  }.
\end{align*}
We can use the subspace separation method to split the transgression
$T_{\mathcal{A}^{g}\leftarrow0}^{\left(  2n+1\right)  }$ as follows%
\begin{equation}
T_{\mathcal{A}^{g}\leftarrow0}^{\left(  2n+1\right)  }=T_{\mathcal{A}%
^{g}\leftarrow g^{-1}dg}^{\left(  2n+1\right)  }+T_{g^{-1}dg\leftarrow
0}^{\left(  2n+1\right)  }+dQ_{\mathcal{A}^{g}\leftarrow g^{-1}dg\leftarrow
0}^{\left(  2n\right)  }. \label{ch2wzw}%
\end{equation}
The right hand side of eq.$\left(  \ref{ch2wzw}\right)  $ can be evaluated
term by term. In fact, the first term corresponds to the Chern--Simons form
$T_{\mathcal{A}\leftarrow0}^{\left(  2n+1\right)  }$, where%
\[
T_{\mathcal{A}^{g}\leftarrow g^{-1}dg}^{\left(  2n+1\right)  }=\left(
n+1\right)  \int_{0}^{1}dt\left\langle g^{-1}\mathcal{A}g\wedge\mathcal{F}%
_{t}^{n}\right\rangle
\]
and $\mathcal{F}_{t}$ is the curvature for the connection $\mathcal{A}_{t}$
given by%
\[
\mathcal{A}_{t}=g^{-1}dg+tg\mathcal{A}g^{-1}.
\]
Using eq.$\left(  {}\right)  $[][][][][] it is direct to show that%
\[
\mathcal{F}_{t}=g^{-1}\left(  td\mathcal{A}+t^{2}\mathcal{A}\wedge
\mathcal{A}\right)  g
\]
and then%
\[
T_{\mathcal{A}^{g}\leftarrow g^{-1}dg}^{\left(  2n+1\right)  }=T_{\mathcal{A}%
\leftarrow0}^{\left(  2n+1\right)  }\text{.}%
\]


Let us now to evaluate the second term in eq.$\left(  \ref{ch2wzw}\right)  $.
Using eq.$\left(  \text{[[[[[[[]]]]]\}}\right)  $\newline%
\begin{align*}
T_{g^{-1}dg\leftarrow0}^{\left(  2n+1\right)  }  &  =\left(  n+1\right)
\int_{0}^{1}dt\left\langle \left(  g^{-1}dg\right)  \wedge\left(  td\left(
g^{-1}dg\right)  +t^{2}\left(  g^{-1}dg\right)  ^{2}\right)  ^{n}\right\rangle
,\\
&  =\left(  n+1\right)  \left(  -1\right)  ^{n}\int_{0}^{1}dtt^{n}\left(
1-t\right)  ^{n}\left\langle \left(  g^{-1}dg\right)  \wedge\left(
g^{-1}dg\right)  ^{2n}\right\rangle ,\\
&  =\left(  -1\right)  ^{n}\frac{n!\left(  n+1\right)  !}{\left(  2n+1\right)
!}\left\langle \left(  g^{-1}dg\right)  \wedge\left(  g^{-1}dg\right)
^{2n}\right\rangle ,
\end{align*}
where we have used%
\[
\int_{0}^{1}dtt^{n}\left(  1-t\right)  ^{n}=\frac{\left(  n!\right)  ^{2}%
}{\left(  2n+1\right)  !}.
\]
This term is the so called Wess--Zumino term and corresponds to a closed,
however not exact, $\left(  2n+1\right)  -$form $dT_{g^{-1}dg\leftarrow
0}^{\left(  2n+1\right)  }=0$. Since the Wess--Zumino term represents a
winding number, it will be a total derivative unless $\mathcal{G}$ has
nontrivial homotopy group $\pi(\mathcal{G})$ and a large gauge transformation
is performed.

The remaining term in eq.$\left(  \ref{ch2wzw}\right)  $ corresponds to%
\[
Q_{\mathcal{A}^{g}\leftarrow g^{-1}dg\leftarrow0}^{\left(  2n\right)
}=-n\left(  n+1\right)  \int_{0}^{1}dt\int_{0}^{t}ds\left\langle
g^{-1}dg\wedge\mathcal{A}\wedge\mathcal{F}_{st}^{n-1}\right\rangle ,
\]
where $\mathcal{F}_{st}=d\mathcal{A}_{st}+\mathcal{A}_{st}\wedge
\mathcal{A}_{st}$, with
\[
\mathcal{A}_{st}=tg^{-1}dg+sg^{-1}\mathcal{A}g.
\]
It is direct to show that
\[
\mathcal{F}_{st}=g^{-1}\left[  s\left(  d\mathcal{A}+s\mathcal{A}%
\wedge\mathcal{A}\right)  +t\left(  1-t\right)  \left(  dgg^{-1}\right)
^{2}\right]  g,
\]
and therefore,%
\[
Q_{\mathcal{A}^{g}\leftarrow g^{-1}dg\leftarrow0}^{\left(  2n\right)
}=-n\left(  n+1\right)  \int_{0}^{1}dt\int_{0}^{t}ds\left\langle
g^{-1}dg\wedge\mathcal{A}\wedge\left[  s\left(  d\mathcal{A}+s\mathcal{A}%
\wedge\mathcal{A}\right)  +t\left(  1-t\right)  \left(  g^{-1}dg\right)
^{2}\right]  ^{n-1}\right\rangle .
\]
Finally, the Chern--Simons Lagrangian $\mathsf{L}_{\mathsf{CS}}^{\left(
2n+1\right)  }\left(  \mathcal{A}^{g}\right)  $, is given by%
\begin{align}
\mathsf{L}_{\mathsf{CS}}^{\left(  2n+1\right)  }\left(  \mathcal{A}%
^{g}\right)   &  =\mathsf{L}_{\mathsf{CS}}^{\left(  2n+1\right)  }\left(
\mathcal{A}\right)  +\left(  -1\right)  ^{n}\frac{n!\left(  n+1\right)
!}{\left(  2n+1\right)  !}\left\langle \left(  g^{-1}dg\right)  \wedge\left(
g^{-1}dg\right)  ^{2n}\right\rangle \nonumber\\
&  -n\left(  n+1\right)  d\int_{0}^{1}dt\int_{0}^{t}ds\left\langle
g^{-1}dg\wedge\mathcal{A}\wedge\left[  s\left(  d\mathcal{A}+s\mathcal{A}%
\wedge\mathcal{A}\right)  +t\left(  1-t\right)  \left(  g^{-1}dg\right)
^{2}\right]  ^{n-1}\right\rangle .\label{ch2csgauge}%
\end{align}
Therefore, the Chern--Simons Lagrangian changes by a closed form under gauge transformations.

We turn now to the transgression Lagrangian eq.$\left(  \ref{ch2tranact}%
\right)  $. In fact inserting eq.$\left(  \ref{ch2csgauge}\right)  $ the
transgression becomes into a gauged Wess--Zumino--Witten Lagrangian%
\begin{align*}
\mathsf{L}_{\mathsf{T}}^{\left(  2n+1\right)  }\left(  \mathcal{A}%
,\mathcal{A}^{g}\right)    & =\mathsf{L}_{\mathsf{gWZW}}^{\left(  2n+1\right)
}\left(  \mathcal{A},\mathcal{A}^{g}\right)  \\
& =\left(  -1\right)  ^{n+1}\frac{n!\left(  n+1\right)  !}{\left(
2n+1\right)  !}\left\langle \left(  g^{-1}dg\right)  \wedge\left(
g^{-1}dg\right)  ^{2n}\right\rangle +d\left(  \alpha^{\left(  2n\right)
}-\beta^{\left(  2n\right)  }\right)
\end{align*}
where $\alpha=\kappa Q_{\mathcal{A}^{g}\leftarrow g^{-1}dg\leftarrow
0}^{\left(  2n\right)  }$ and $\beta=\kappa Q_{\mathcal{A}\leftarrow
\mathcal{A}^{g}\leftarrow0}^{\left(  2n\right)  }$.

This Lagrangian has interesting properties. For instance, the $n=1$ case
conduces to a gauged Wess--Zumino--Witten action given by%
\[
\mathsf{S}_{\mathsf{gWZW}}\left[  \mathcal{A},g\right]  =\kappa\int
_{\mathcal{M}}\frac{1}{3}\left\langle \left(  g^{-1}dg\right)  ^{3}%
\right\rangle +d\left\langle 2\left(  g^{-1}dg\right)  \wedge\mathcal{A+A}%
g^{-1}\wedge\mathcal{A}g\right\rangle .
\]
If we consider the action valued in the Poincare group $ISO(2,1)$, this model
corresponds to a boundary term. In the next chapter, we will show that the
resulting Wess--Zumino--Witten action in two dimensions is the simplest
version for a topological action for gravity in even dimensions classified in
ref\{\}\{\}. Furthermore, the two dimensional Wess--Zumino--Witten model is
conformal invariant and corresponds to the asymptotically flat limit of the
conformal field theory holographically dual to the three dimensional
Chern--Simons gravity action genuinely invariant under the anti--de Sitter
group $SO(2,2)$. 
